Pose Forecasting in Industrial Human-Robot Collaboration

Pushing back the frontiers of collaborative robots in industrial environments, we propose a new Separable-Sparse Graph Convolutional Network (SeS-GCN) for pose forecasting. For the first time, SeS-GCN bottlenecks the interaction of the spatial, temporal and channel-wise dimensions in GCNs, and it learns sparse adjacency matrices by a teacher-student framework. Compared to the state-of-the-art, it only uses 1.72% of the parameters and it is ~4 times faster, while still performing comparably in forecasting accuracy on Human3.6M at 1 second in the future, which enables cobots to be aware of human operators. As a second contribution, we present a new benchmark of Cobots and Humans in Industrial COllaboration (CHICO). CHICO includes multi-view videos, 3D poses and trajectories of 20 human operators and cobots, engaging in 7 realistic industrial actions. Additionally, it reports 226 genuine collisions, taking place during the human-cobot interaction. We test SeS-GCN on CHICO for two important perception tasks in robotics: human pose forecasting, where it reaches an average error of 85.3 mm (MPJPE) at 1 sec in the future with a run time of 2.3 msec, and collision detection, by comparing the forecasted human motion with the known cobot motion, obtaining an F1-score of 0.64.

==> addmat/Actions.tex <==
\newpage
\section{The CHICO Dataset}
\label{sec:chico_viz}

Here we illustrate additional details on the scenario of the dataset and the acquisition process; furthermore,  we report a graphical explanation of all the 8 actions.
For further details, please watch the additional video, enclosed in \url{https://github.com/AlessioSam/CHICO-PoseForecasting}.


\subsection{Details on the dataset and the data acquisition process}
The dataset has been acquired in the October '21 - March '22 period, on a $500m^2$ Industry 4.0 lab, which includes a configurable a 11m production line, 4 cobots, a quality inspection cell, a (dis-)assembly station and other equipment. We worked on the 0.9 m ×0.6 m workbench of the (dis-)assembly station in front of a  Kuka LBR iiwa 14 R820 cobot. The declared positioning accuracy is $\pm \SI{0.1}{mm}$ and the axis-specific torque accuracy is $\pm \SI{2}{\%}$~\cite{kuka_manual}. Thanks to its joint torque sensors, the robot can detect contact and reduce its level of force and speed, being compliant to the ISO/TS 15066:2016~\cite{iso15066} standard. Since collisions between the operator and the cobot were expected in \dataname{}, the maximum allowed Cartesian speed of each link is set to $\SI{200}{mm/s}$, slightly lower than the ISO/TS 15066:2016 requirements. The safety torque limit allowed before the mechanical brakes activation is set to $\SI{30}{\newton\meter}$ for all joints and $\SI{50}{\newton\meter}$ for the end-effector. Additionally, a programmable safety check of $\SI{10}{\newton}$ was set on the Cartesian force. %The operator safety was guaranteed by covering the end-effector with bubble wrap layers, as seen in Figure~\ref{fig:video_frames}. For added safety, a second human operator with access to hand-held switches was always present during the recording sessions.\MC{Bisogna spiegare come abbiamo fatto ad acquisire il robot, e come l'abbiamo sincronizzato nel tempo e nello spazio con la persona!}
%\subsection{Actions} \label{subsec:actions}

A total of 20 subjects (14 males, 6 females, average age 23 years) have been hired for building the dataset. They worked for the entire acquisition period, after having signed an informed consent and participated on a crash course on how to cooperate with the Kuka cobot. During the acquisition season, we have selected some excerpts which capture collisions made by the operators, reaching 226 collisions.
In average we have 45 collisions for each action, with the sole exception for \textit{hammering}. For this specific action, the cobot stands still, holding the object being hammered, while the human agent moves repeatedly close to the robotic arm.
Sequences containing this action are still part of the collision detection dataset, i.e.\ they are useful to check that there are no false positives.
%In average we have 22 collisions per action, apart the hammering action: in that case, the robot was still, holding the object to be hammered, so no collisions took place. Still, the hammering action was interesting to check for false positive collisions, since the action required the human operator to move close to the robotic arm.  
%Recall that the task of detection is test-only, i.e.\ models train on collision-less excerpts and should be capable of extrapolating the motion to detect collisions.

%\newpage
\subsection{Details on the actions}
In this section we expand the short explanations of each action given in Sec.4 of the main paper. For each action, we report the original description, and a detailed graphical storyboard. 


%-------------------- 1 -------------------
\begin{itemize}
    \item \emph{\textbf{Lightweight pick and place}} (\emph{Light P\&P}). The human operator is required to move small objects of approximately 50 grams from a loading bay to a delivery location within a given time slot. The bay and the delivery location are at the opposite sides of the workbench. 
    Meanwhile, the robot loads on of this bay 
    so that the human operator has to pass close to the robotic arm.
    In many cases the distance between the limbs and the robotic arm is few centimeters. 

 %\begin{figure}[H]
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
    \includegraphics[width=1.0\linewidth]{addmat/fig/1.pdf}
    \caption{\emph{\textbf{Lightweight pick and place}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''.  A single item (the red brick) is showed here for clarity. In practice, a dozen of items was available.%, where the small objects are moved from loading bay B2 to delivery location 10 by the robot (steps 1-3)\MC{inserire graficamente gli step}, and brought back by the human to the delivery location (steps 4-6)
    }
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}
\end{itemize}
\newpage
%-------------------- 2 -------------------
\begin{itemize}
    \item \emph{\textbf{Heavyweight pick and place}} (\emph{Heavy P\&P}). The setup of this action is the same as before, but the objects to be moved are floor tiles weighing $\SI{0.75}{\kilogram}$.
    %\footnote{Fix: in the main paper it was written $\SI{0.25}{\kilogram}$}. 
    This means that the actions have to be carried out with two hands. %Collisions were mostly on the external parts of the right forearm, in few cases with the left wrist.
\end{itemize}
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
  \includegraphics[width=1.0\linewidth]{addmat/fig/2.pdf}
    \caption{\emph{\textbf{Heavyweight pick and place}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''.
    Moving the object with two hands requires to strongly rotating the torso, and this partially hides the robot from the operator, being back to him/her. This was the main cause of the collisions occurred with this action.}
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}
\newpage
%-------------------- 3 -------------------
\begin{itemize}
     \item \emph{\textbf{Surface polishing}} (\emph{Polishing}). This action was inspired by~\cite{magrini2020human}, where the human operator polishes the border of a 40 by 60cm tile with some abrasive sponge, and the robot mimics a visual quality inspection.
     
\end{itemize}
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
  \includegraphics[width=1.0\linewidth]{addmat/fig/3.pdf}
    \caption{ \emph{\textbf{Surface polishing}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''. The human has an abrasive sponge used to remove some material from the metallic tile. This action created most of the collisions,  since the action required the user to be prone on the surface to polish, blocking the view of the robot.}
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}
\newpage

%-------------------- 4 -------------------
\begin{itemize}
     \item \emph{\textbf{Precision pick and place}} (\emph{Prec. P\&P}). The robot places four plastic pieces in the four corners of a 30$\times$30cm table in the center of the workbench, and the human has to remove them and put on a bay, before the robot repeats the same unloading. %This action was
\end{itemize}
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
  \includegraphics[width=1.0\linewidth]{addmat/fig/4.pdf}
    \caption{\emph{\textbf{Precision pick and place}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''. This action is important, since it allows to measure how precise the prediction could be in individuating particular endpoints which will be targeted by the human operator.}
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}
\newpage
%-------------------- 5 -------------------
\begin{itemize}
    \item \emph{\textbf{Random pick and place}} (\emph{Rnd. P\&P}). Same as the previous action, except for the plastic pieces which were continuously placed by the robot randomly on the central 30$\times$30cm table, and the human operator has to remove them. %This 
\end{itemize}
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
  \includegraphics[width=1.0\linewidth]{addmat/fig/5.pdf}
    \caption{\emph{\textbf{Random pick and place}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''. The action is interesting, since the robot puts objects randomly on the workplace, and this created some collisions during the interaction. A single item (the red brick) is showed here for clarity. In practice, a dozen of items was available.}
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}
\newpage
%-------------------- 6 -------------------
% \begin{itemize}
%      \item \emph{\textbf{Lifting from the floor}} (\emph{Low lift}). %From this action on, human and robot share their space, so no collision was recorder. Nonetheless, human and robot stay very close, so that the challenge here is to avoid false positive collisions. 
%     In this case, rectangular tiles were lifted from the floor to the workbench, where the robot is picking them in the meanwhile. %In
% \end{itemize}
%  \begin{figure}[H]
%     \centering
%     % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
%   \includegraphics[width=1.0\linewidth]{addmat/fig/6.pdf}
%     \caption{\emph{\textbf{Lifting from the floor}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''. This action is interesting since the movement of the person has a strong torsion, and has some vertical dynamics (from the floor to the workbench), since the operator has to crouch to take the tile.}
%     \label{fig:span_light}
%   %\vspace{-0.5cm}
% \end{figure}
% \newpage
%-------------------- 7 -------------------
\begin{itemize}
   \item \emph{\textbf{High shelf lifting}} (\emph{High lift}). The goal was to pick light plastic pieces (50 grams each) on a sideway bay filled by the robot, putting them on a shelf located at 1.70m, at the opposite side of the workbench. Due to the geometry of the workspace, the arms of the human operator were required to pass above or below the moving robotic arm.    In this way, close distances between the human arm and forearm and the robotic links were realized. 
\end{itemize}
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
  \includegraphics[width=1.0\linewidth]{addmat/fig/7.pdf}
    \caption{\emph{\textbf{High shelf lifting}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''.}
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}
\newpage
%-------------------- 8 -------------------
\begin{itemize}
    \item \emph{\textbf{Hammering}} (\emph{Hammer}). The operator hits with a hammer a metallic tide held by the robot. In this case, the interest was to check how much the collision detection is robust to an action where the human arm is colliding close to the robotic arm (that is, on the metallic tile) without properly colliding \emph{with the robotic arm}.
\end{itemize}
 \begin{figure}[H]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
  \includegraphics[width=1.0\linewidth]{addmat/fig/8.pdf}
    \caption{\emph{\textbf{Hammering}} illustration; ``\emph{\textbf{H}}'' stands for ``human operator'', ``\emph{\textbf{R}}'' for ``robot''. This action is important since it tests the collision prediction task against false positive alarms. In facts, this action requires the human to be very close to the robot, keeping the item to hammer with one hand, the other doing the hammering action. In facts, this action was creating the most false positive alarms, around 80\%.}
    \label{fig:span_light}
   %\vspace{-0.5cm}
\end{figure}

==> addmat/implementation_details.tex <==
%\newpage
\section{Implementation and Learning}
\label{sec:impl_det}

Further to what included in Secs.~3 and 5 \textit{(main paper)}, we 
discuss here a few additional details on implementation and learning.


\subsection{Implementation details}
The proposed SeS-GCN is written in Pytorch (the source code will be distributed).
The model adopts residual connections at each GCN layers, it is regularized with batch normalization~\cite{batchnorm15} at the end of each GCN layer, and it is optimized with ADAM~\cite{adam15}.

\subsection{Learning time}
On Human3.6M~\cite{h36m_pami}, training of SeS-GCN proceeds for 60 epochs for both the teacher and the student models. We used batch size of 256, learning rate of 0.1, and decay rate of 0.1 at epochs 5, 20, 30 and 37.
On an Nvidia RTX 2060 GPU, the learning process takes 30 minutes.

\subsection{Loss function}

Following literature~\cite{Mao19LTD,Mao20DCT,Dang21}, the loss function differs from the test metric, Eq.~(5) main paper; namely, the loss function considers the average of MPJPEs over the entire predicted sequence:
\begin{equation*}
    L_{\text{MPJPE}}= \frac{1}{VT} \sum_{t=0}^{T} \sum_{v=1}^{V}||\hat{\boldsymbol{x}}_{vt}-\boldsymbol{x}_{vt} ||_{2}
\end{equation*}
where, in accordance with Eq.~(5), $\hat{\boldsymbol{x}}_{vt}$ and $\boldsymbol{x}_{vt}$ are the 3-dimensional vectors of a target joint $j_v\ (0\leq v \leq V)$ in a fixed frame $f_t\ (0 \leq t \leq T)$ for the ground truth and the predictions, respectively.


\begin{figure}[t]
    \centering

    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
    \includegraphics[width=1\linewidth, height=0.56\linewidth]{addmat/fig/pipeline.pdf}
    \caption{Overview of the proposed pipeline. Given a sequence of observed 3D poses, the Teacher network (depicted with blue boxes) encodes the spatio-temporal body dynamics with 5 SeS-GCN layers, composed by the space-time separable encoder followed by the Depth-Wise convolution. The future trajectories are then predicted with 4 TCN layers. After the train of the Teacher, we threshold the values of the spatial and temporal adjacency matrix to obtain the masks which are then applied during the Student model (depicted in orange boxes) training.}
    %We perform a sparsification of the learned adjacency matrices, and the generated mask is given as input to the Student network. As the second stage, the model encodes the input and masks, then generates future predictions of the human pose as for the Teacher network.} %\TD{14 out of 17 joints are represented for better view}.
    \label{fig:error}
   %\vspace{-0.5cm}
\end{figure}
%\subsection{Runtime}
%Table 5 \textit{(main paper)} illustrates runtimes for the best performing pose forecasting techniques, against which SeS-GCN is benchmarked (cf.\ performance evaluation in Tables 2 and 4\textit{(main paper)}).

%Both STS-GCN~\cite{stsgcn} and the proposed SeS-GCN are fast, almost 4x times faster than the competing DCT-RNN-GCN~\cite{Mao20DCT} and more than 10x times faster than MSR-GCN~\cite{Dang21}.

%While runtime of STS-GCN~\cite{stsgcn} and the proposed SeS-GCN is almost the same, SeS-GCN achieves a lower error over all the tested datasets. Overall, this is explainable as the benefit of the increased depth of SeS-GCN (10 layers Vs 4 of STS-GCN), achieved with nearly the same parameter count as STS-GCN.

%\FG{Not clear what is the aim of this subsection. We should not add further comments on the material in main paper. Rather we may add runtimes for other techniques such as those in Table 2 and 3 (main paper). However we had discussed that two runtimes for the same techniques would be tricky (but informative) to explain.  So maybe remove this entire subsection altogether.}

==> addmat/quantitative_results.tex <==
\section{Additional Quantitative Results}
\label{sec:amass3dpw}

First we report further experimental evaluation of SeS-GCN on the dataset AMASS~\cite{AMASS:ICCV:2019}, adopting the standard Mean Per-Joint Position Error metric (MPJPE). Then we report angular error evaluations on Human3.6M~\cite{h36m_pami}, using the Mean Angular Error (MAE).


%including angular error evaluations on Human3.6M~\cite{h36m_pami}, and the MPJPE errors on two additional datasets for pose forecasting: AMASS~\cite{AMASS:ICCV:2019} and 3DPW~\cite{vonMarcard2018}.
%The proposed SeS-GCN, thanks to its structure optimized to encode human movements, still results the most efficient model in terms of both performance and inference times.


\subsection{AMASS}


The AMASS~\cite{AMASS:ICCV:2019} dataset contains actions which substantially differ from the work of a human agent at an industrial production assembly line. In view of space constraints in the main paper, the results are  therefore only reported in this supplemental material.
Following the protocols of \cite{stsgcn,Mao20DCT}, the AMASS results are reported for the test subset AMASS-BMLrub.%, while the entire 
%\AS{solo test set} 
% 3DPW is used as a sole test set (models are trained on the training set of AMASS). %\FG{Please review my statement}

%AMASS is a dataset for human pose forecasting approximately 14 times larger than H3.6M \cite{Aksan_2019_ICCV}. This vastness of data is due to the fact
% lo so è terribile, ma non mi veniva un'altra frase...
%that AMASS turns out to be a collection of heterogeneous datasets that contain a wide variety of different activities, from simple \textit{walking} to more challenging poses such as \textit{dancing} or \textit{fancing}. Although the actions in the industrial process are much less articulated than those in this dataset, we benchmarked SeS-GCN to assess its ability to produce credible poses even in this broad scenario.


In Table~\ref{tab:amass}, results show that SeS-GCN outperforms DCT-RNN-GCN~\cite{Mao20DCT} and are competitive with STS-GCN~\cite{stsgcn}, which confirms the robustness of the proposed technique.


\input{addmat/tab/amass}



\subsection{Angular error on Human3.6M}

% \FG{check across this document that Human3.6M is written so, not H3.6M, or h3.6M. Similarly check conistent names for SeS-GCN, STS-GCN, MSR-GCN, etc.} \GD{ho controllato qui non vedo ambiguità}

Following the protocol of \cite{Julieta17,stsgcn,Mao20DCT,Mao19LTD},  
%\FG{give some citations of methods reporting MAE}, 
we consider the Euler angle %angular \FG{Euler? please check} 
representation of joints for the Human3.6M dataset~\cite{h36m_pami} and report the Mean Angular Errors (MAE).
Note that most recent literature~\cite{Dang21,Mao20DCT,stsgcn} mainly refers to MPJPE as metric. 
MAE is strongly criticized in \cite{Akhter_2015_CVPR} and in \cite{Cai20}.

In Table \ref{tab:ang_full}, we compare the proposed SeS-GCN against the state-of-the-art techniques of
STS-GCN~\cite{stsgcn} and DCT-RNN-GCN~\cite{Mao20DCT}.
Consistently with MPJPE, SeS-GCN is the top performer on the short- and long-term predictions.
%in the joint angles format and tested the proposed SeS-GCN in this representation to evaluate its robustness to the different ways the input can be encoded. Consistently with what happens with 3d joint positions, our model maintains primacy even in this different format, showing itself capable of learning to distinguish the spatial and temporal relations peculiar to human motion, heedless of the specific encoding.

\input{addmat/tab/ALL_ANG}



==> addmat/tab/ALL_ANG.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{}                    & \multicolumn{2}{c|}{Walking}             & \multicolumn{2}{c|}{Eating}              & \multicolumn{2}{c|}{Smoking}             & \multicolumn{2}{c|}{Discussion}          & \multicolumn{2}{c|}{Directions}          & \multicolumn{2}{c|}{Greeting}            & \multicolumn{2}{c|}{Phoning}             & \multicolumn{2}{c|}{Posing}              \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}}      & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}        & 0.71               & 1.03                & 1.20               & 1.31                & 1.23               & 1.50                & 1.25               & 1.82                & 1.30               & 1.42                & 1.38               & 1.99                & 1.07               & 1.76                & 1.22               & 2.24                \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}            & \textbf{0.55}               & 0.87                & 0.53               & 1.03                & 0.53               & 1.04                & 0.84               & 1.37                & 0.55               & 1.03                & 0.94               & 1.44                & 0.70               & 1.19                & 0.76               & 1.45                \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)} & \textbf{0.55}      & \textbf{0.86}       & \textbf{0.52}      & \textbf{0.91}       & \textbf{0.52}      & \textbf{0.98}       & \textbf{0.82}      & \textbf{1.30}       & \textbf{0.54}      & \textbf{0.97}       & \textbf{0.92}      & \textbf{1.42}       & \textbf{0.68}      & \textbf{1.16}       & \textbf{0.74}      & \textbf{1.42}       \\ \hline
\end{tabular}}
\label{tab:ang_all1}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{}                              & \multicolumn{2}{c|}{Purchases}           & \multicolumn{2}{c|}{Sitting}             & \multicolumn{2}{c|}{Sitting Down}        & \multicolumn{2}{c|}{Taking Photo}        & \multicolumn{2}{c|}{Waiting}             & \multicolumn{2}{c|}{Walking Dog}         & \multicolumn{2}{c|}{Walking Together}    & \multicolumn{2}{c|}{Average}             \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}                  & 1.32               & 1.82                & 1.06               & 1.88                & 1.39               & 2.22                & 0.72               & 1.33                & 1.07               & 1.77                & 1.12               & 1.63                & 0.71               & 1.04                & 1.04               & 1.65                \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}                      & \textbf{0.94}      & 1.41                & 0.68               & 1.29                & 0.93               & 1.63                & 0.47               & 1.02                & 0.66               & 1.24                & 0.83               & 1.25                & \textbf{0.50}               & 0.83                & 0.69               & 1.21                \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}           & \textbf{0.94}      & \textbf{1.36}       & \textbf{0.67}      & \textbf{1.22}       & \textbf{0.90}      & \textbf{1.53}       & \textbf{0.46}      & \textbf{0.88}       & \textbf{0.64}      & \textbf{1.18}       & \textbf{0.81}      & \textbf{1.22}       & \textbf{0.50}      & \textbf{0.81}       & \textbf{0.68}      & \textbf{1.15}       \\ \hline
\end{tabular}}
\caption{Mean Angular Errors (MAE) of short- and long-term predictions on Human3.6M \cite{h36m_pami}. SeS-GCN achieves the lowest error.}
\label{tab:ang_full}
\end{table*}

==> addmat/tab/Backup/quant_bk_2022-03-13.tex <==
\section{Additional Quantitative Results}
\label{sec:amass3dpw}
Here we report further material to supplement the experimental evaluation of SeS-GCN in the \textit{(main paper)}. This section complements the exposed results by showing the performance of SeS-GCN in the angular representation of the H36M \cite{h36m_pami} dataset and on two more challenging and well-established datasets: AMASS \cite{AMASS:ICCV:2019} and 3DPW \cite{vonMarcard2018}. The proposed SeS-GCN, thanks to its structure optimized to encode human movements, still results the most efficient model in terms of both performance and inference times.


\subsection{Angular error on Human3.6M}
We extracted the same data as H3.6M in the joint angles format and tested the proposed SeS-GCN in this representation to evaluate its robustness to the different ways the input can be encoded. Consistently with what happens with 3d joint positions, our model maintains primacy even in this different format, showing itself capable of learning to distinguish the spatial and temporal relations peculiar to human motion, heedless of the specific encoding.

\input{addmat/tab/ang_error}

\subsection{Amass and 3DPW} AMASS is a dataset for human pose forecasting approximately 14 times larger than H3.6M \cite{Aksan_2019_ICCV}. This vastness of data is due to the fact
% lo so è terribile, ma non mi veniva un'altra frase...
that AMASS turns out to be a collection of heterogeneous datasets that contain a wide variety of different activities, from simple \textit{walking} to more challenging poses such as \textit{dancing} or \textit{fancing}. Although the actions in the industrial process are much less articulated than those in this dataset, we benchmarked SeS-GCN to assess its ability to produce credible poses even in this broad scenario. Table \ref{tab:amass} shows that SeS-GCN significantly improves the performance of DCT-RNN-GCN \cite{Mao20DCT} while achieving comparable results with STS-GCN \cite{stsgcn}, improving the previous SoA by XX\%. We evaluated on the AMASS-BMLrub subset following the field literature [A, B, C], which has the same fps as 3DPW and H3.6M. 
%Aggiungere dettagli su 3dpw
\input{addmat/tab/amass}




==> addmat/tab/amass.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


% \begin{table}[!h]
% \centering
% \begin{tabular}{c|cc|cc|}
% \cline{2-5}
% \multicolumn{1}{l|}{}                             & \multicolumn{2}{c|}{AMASS}               & \multicolumn{2}{c|}{3DPW}                \\ \hline
% \multicolumn{1}{|l|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
% \multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}                 & 42.0               & 67.2                & 45.4               & 73.7                \\
% %\multicolumn{1}{|c|}{MSR-GCN\cite{Dang21}}                      & ---                & ---                 & ---                & ---                 \\
% \multicolumn{1}{|c|}{STS-GCN\cite{stsgcn}}                     & \textbf{24.5}               & 45.5                & \textbf{24.5}               & \textbf{42.3}                \\ \hline
% \multicolumn{1}{|c|}{SeS-GCN (proposed)}          &         24.9           &         \textbf{45.2}            &      \textbf{24.5}              &       42.5              \\ \hline
% \end{tabular}
% \caption{MPJPE on short- and long-term prediction on AMASS and 3DPW.}
% \label{tab:amass}
% \end{table}

\begin{table}[!h]
\centering
\begin{tabular}{c|cc|}
\cline{2-3}
\multicolumn{1}{l|}{}                                              & \multicolumn{2}{c|}{AMASS}                                    \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}}                          & \multicolumn{1}{c|}{{\ul \textit{400}}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}} & \multicolumn{1}{c|}{42.0}               & 67.2                \\ \hline
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & \multicolumn{1}{c|}{\textbf{24.5}}      & 45.5                \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}                           & \multicolumn{1}{c|}{24.9}               & \textbf{45.2}       \\ \hline
\end{tabular}
\caption{MPJPE on short- and long-term prediction on AMASS.}
\label{tab:amass}
\end{table}

==> addmat/tab/ang_error.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[!h]
\centering
\begin{tabular}{c|cc|}
\cline{2-3}
\multicolumn{1}{l|}{}                             & \multicolumn{2}{c|}{Human3.6M}           \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (millisec)}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}                 & 1.04               & 1.65                \\
\multicolumn{1}{|c|}{MSR-GCN\cite{Dang21}}                      & ---                & ---                 \\
\multicolumn{1}{|c|}{STS-GCN\cite{stsgcn}}                     & 0.69               & 1.21                \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}          & \textbf{0.68}                   &  \textbf{1.15}                   \\ \hline
\end{tabular}
\caption{Mean Angular Errors (MAE) of short- and long-term predictions on Human3.6M \cite{h36m_pami}. SeS-GCN achieves the lowest error. \FG{Missing MSR-GCN? if so one may explain why in the next but do not report an empty line here.} \AS{MSR non riporta mai i risultati in angoli nel suo paper}}
\label{tab:mae}
\end{table}

==> src/Backup/abs_bk_2022-03-05.tex <==

\begin{abstract}
Adhering to the field of Human Robot Collaboration (HRC), we propose a new pose forecasting model dubbed \gcnname{}: Separable Sparse Graph Convolutional Network, which complies with all the requirements that HRC asks: high accuracy in the prediction, and fast inference. \gcnname{}{} is a novel ``fully-separable'' type of GCN, that is the first to bottleneck all the spatial, temporal and channel-wise dimensions of a GCN, by learning sparsified adjacency matrices.  \gcnname{}{} is effective on modern human pose forecasting datasets, improving SoA accuracy by 3.6\% on Human3.6M on long-term prediction horizons while using 14.5\% less parameters. As a second contribution, we present a new dataset focused on Cobots and Humans in Industrial COllaboration, \dataname{}, which includes 3D pose and trajectories of 8 human operators and cobots while interacting during 8 realistic industrial tasks. As unique feature, \dataname{} contains 158 genuine collisions between the operators and the cobots, so that forecasting can be exploited to foresee what a human is about to do, anticipating the collisions with the robot.  On \dataname{}, \gcnname{} reaches an average error of 57.3mm (MPJPE) at 1.6sec in the future, anticipating collisions with XX as precision and YY as recall. Collisions in the datasets were harmless for the human operators.
%opening a novel research frontier for HRC, where the robot anticipates what a human is about to do for a faster and seamless interaction.
\\
%\MC{cambia acronimo} \FG{Industrial Human Cobot Interaction (InHCI) dataset}\\
%\FG{Industrial Human Cobot Collaboration (IHCoCo) dataset}
\end{abstract}




%%%%% below the bits and pieces
% Towards the frontier of collaborative robots in industrial environments, 
% we propose a new Separable-Sparse Graph Convolutional Network (\gcnname) for pose forecasting.
% For the first time, \gcnname{} bottlenecks the interaction of the spatial, temporal and channel-wise dimensions in GCNs, and it learns sparse adjacency matrices by a teacher-student framework. It improves the state-of-the-art by 3.6\% on Human3.6M on long-term predictions, it reduces the number of parameters by 14.5\%, and it effectively predicts human motion at 1 second in the future with a negligible 5 msec processing time.

% As a second contribution, we present a new benchmark of Cobots and Humans in Industrial COllaboration (\dataname{}).
% \dataname{} includes multi-view images, 3D poses and trajectories of 8 human operators and cobots, engaging in 8 realistic industrial actions. Additionally, it reports 158 genuine collisions, taking place during the human-cobot interaction.
% We test \gcnname{} on \dataname{} for two important perception tasks for robotics: human pose forecasting, where it reaches an average error of 57.3mm (MPJPE) at 1.2 sec in the future, and collision detection, by means of comparing the forecast human motion with that of the cobot, for which it yields an F1-score of X.



% We test \gcnname{} on \dataname{} for two important perception tasks for robotics: it yields human pose forecasting at an average error of 57.3mm (MPJPE) at 1.2 sec in the future, and 

% \gcnname{} reaches an average error of 57.3mm (MPJPE) at 1.2 sec in the future


% We test on \dataname{} two important perception goals for robotics: human pose forecasting and collision detection.
% This is a novel benchmark for two important perception goals 

% As unique feature, \dataname{} contains 158 genuine collisions between the operators and the cobots, so that forecasting can be exploited to foresee what a human is about to do, anticipating the collisions with the robot.  On \dataname{}, \gcnname{} reaches an average error of 57.3mm (MPJPE) at 1.2 sec in the future, anticipating collisions with XX as precision and YY as recall. Collisions in the datasets were harmless for the human operators.

% For the first time, \gcnname{} brings together depthwise-separable graph convolutions, space-time-separable graph convolutional networks (GCN), and sparsity. \gcnname{} bottlenecks the interaction of spatial, temporal and channel-wise dimensions and it learns sparse adjacency matrices by teacher-student frameworks. So it improves the state-of-the-art by 3.6\% on Human3.6M on long-term predictions, it reduces the number of parameters by 14.5\%, and it effectively predicts at more than 1 second in the future with a negligible 5 msec processing time.

% As a second contribution, we present a new dataset focused on Cobots and Humans in Industrial COllaboration (\dataname{}) which includes multi-view images, 3D poses and trajectories of 8 human operators and cobots while interacting during 8 realistic industrial tasks.
% As unique feature, \dataname{} contains 158 genuine collisions between the operators and the cobots, so that forecasting can be exploited to foresee what a human is about to do, anticipating the collisions with the robot.  On \dataname{}, \gcnname{} reaches an average error of 57.3mm (MPJPE) at 1.2 sec in the future, anticipating collisions with XX as precision and YY as recall. Collisions in the datasets were harmless for the human operators.


% is a novel ``fully-separable'' type of GCN, that is the first to bottleneck all the spatial, temporal and channel-wise dimensions of a GCN, by learning sparsified adjacency matrices.  \gcnname{}{} is effective on modern human pose forecasting datasets, improving SoA accuracy by 3.6\% on Human3.6M on long-term prediction horizons while using 14.5\% less parameters.

% \gcnname complies with all the requirements of Human-Robot Collaboration (HRC) tasks: high accuracy in the prediction, and fast inference





==> src/Backup/abs_bk_2022-03-07.tex <==

\begin{abstract}
Towards the frontier of collaborative robots in industrial environments, 
we propose a new Separable-Sparse Graph Convolutional Network (\gcnname) for pose forecasting.
For the first time, \gcnname{} bottlenecks the interaction of the spatial, temporal and channel-wise dimensions in GCNs, and it learns sparse adjacency matrices by a teacher-student framework. It improves the state-of-the-art by 3.6\% on Human3.6M on long-term predictions with a competing parameter count, and it effectively predicts human motion at 1 second in the future with a negligible 5 msec \MC{inserire runtime su chico} run time, unleashing the cobot awareness.

As a second contribution, we present a new benchmark of Cobots and Humans in Industrial COllaboration (\dataname{}).
\dataname{} includes multi-view videos, 3D poses and trajectories of 20 human operators and cobots, engaging in 8 realistic industrial actions. Additionally, it reports 158 genuine collisions, taking place during the human-cobot interaction.
We test \gcnname{} on \dataname{} for two important perception tasks for robotics: human pose forecasting, where it reaches an average error of 53.0mm (MPJPE) at 1.25 sec in the future, and collision detection, by means of comparing the forecast human motion with that of the cobot\MC{WARNING: we don't do a proper robot forecasting, since we know where it will go FABIO}, for which it yields an F1-score of \MC{X}.

\keywords{Human Pose Forecasting,  Graph Convolutional Network, Human-Robot Collaboration in Industry.}

\end{abstract}

==> src/Backup/bg_bk_2022-03-05.tex <==

%\subsection{Human pose forecasting}
\smallskip
\myparagraph{Human pose forecasting.}
Human pose forecasting is a recent field which has some intersection with human action anticipation in CV~\cite{li20} and HRC~\cite{duarte2018action}. Previous studies exploited architectures like Temporal Convolutional Networks (TCNs) ~\cite{pavllo19,Bai18TCN,Gehring17,Li18} and Recurrent Neural Networks (RNNs)~\cite{fragkiadaki15,jain16,anand19}. Both architectures are naturally suited to model the temporal dimension, in particular RNNs, even though TCNs have been reported to be sable than RNNs. Recent studies have expanded the range of available methods by using Variational Auto-Encoders~\cite{Btepage2017AnticipatingMF} or specific, model-agnostic layers that implicitly model the spatial structure of the human skeleton~\cite{Aksan_2019_ICCV}.

%\textbf{Pose forecasting using Graph Convolutional Networks (GCN)}
\smallskip
\myparagraph{Pose forecasting using Graph Convolutional Networks (GCN).}
represents a consistent body of research~\cite{Zhao20,li21,Dang21,Mao20DCT}. These models are able to process both the spatial and temporal features of the input. Specifically,~\cite{Dang21} predicts future positions leveraging predictions of aggregations of joints that are both informative and easier to predict. In~\cite{Mao20DCT} attention is used to refer to past poses and more recent observations, leveraging the repetitions that some actions may exhibit. These methods require an additional computational effort that can be minimized. Efficiency for GCNs has only emerged recently, with three promising directions: separable convolutions~\cite{chollet17,howard17}, factorization~\cite{stsgcn,berta21} and sparsification~\cite{shi21} of the adjacency matrix. Separable convolutions~\cite{chollet17,howard17} are efficient operations explicitly defined for graph structures in~\cite{lai18}, also applied in~\cite{balcilar20} to the spectral domain. We are the first to apply them in the context of pose forecasting. Factorization of space-time entanglement is a topic studied in diverse domains~\cite{stsgcn,berta21}; notably, it helps the model inference by eliminating the space-time cross-talk. Sparsity has been used to represent interactions among pedestrians in~\cite{shi21}, by iteratively learning a mask on active elements of adjacency matrices. In~\cite{stsgcn}, authors applied sparsity on the learned representations of the spatial and temporal connections, highlighting natural correlations among joints and time steps. To the best of our knowledge, these three aspects have been studied separately and this work is the first to bring these techniques into a single framework. \FG{Cf earlier reviews. We must better spell out the differences between ours and sts-gcn / sgcn. Use text from our rebuttal.}

\smallskip
\myparagraph{Human Robot Collaboration.}
%\FG{From how it reads, it seems pose estimation and collision avoidance are indeed THE tasks to address, which makes sense. So worth saying, at the very first line, "these are the tasks which matter most now, but no dataset is available". However, apart from this sentence (which actually relates to Sec 2.3), this subsection needs to spell out how we relate to HRC, which is currently missing.}\MC{CHecked, going to solve by shuffling the ordering of the subsections, rewriting some parts.}\\
Human Robot Collaboration is the study of collaborative processes where human and robot agents work together to achieve shared goals~\cite{bauer2008human}. Computer vision studies on HRC are mostly related to pose estimation~\cite{OpenPoseTPAMI19,Sarafianos2016,Tan2010,Beckert2018,Araiza-Lllan2018,Lemmerz2019,Garcia-Esteban2021} and motion planning with collision avoidance~\cite{Chen2018,Kanazawa2019,Nascimento2020,Beltran2018,Kang2019,Costanzo2020,Lim2021}. Other subjects are head pose estimation~\cite{patacchiola2017head} and gesture recognition~\cite{liu2018gesture}. In relation to pose estimation, we highlight ~\cite{Tan2010,Beckert2018,Araiza-Lllan2018,Lemmerz2019}, where pose estimation approaches are specifically designed to monitor HR collaboration. In~\cite{Chen2018,Kanazawa2019,Nascimento2020}, methodologies for robot motion planning and collision avoidance are proposed; this represents the point of view opposite to ours, sin ce we focus on the human operator. In~\cite{Beltran2018,Kang2019,Costanzo2020,Lim2021} the operators' whereabouts is obtained through detection algorithms which approximate human shapes using simple bounding boxes. Motion prediction on collaborative tasks have been considered focusing solely on the human counterpart in~\cite{torkar2019rnn,zhang2020recurrent} using RNNs and in~\cite{vianello2021human} using Guassian processes, while~\cite{laplaza2021attention} explicitly modeled the robot end-effector position on specific handover interactions, exploiting DCT-RNN-GCN~\cite{Mao20DCT} as inference engine, with which we compare against in the experiments. 
Notably, in all of the above quoted cases, no datasets have been provided, as we do. More importantly, we are the first in considering and predicting collisions in a HRC context, on a various set of actions.   

%Notably, we are the first in proposing human pose forecasting in a HRC context,  \emph{providing the first dataset taken in an industrial setup, equipped with HR collisions}, plus associated baselines, to promote further research.
%\FG{emphasize common and distinct aspects, distinguishing: (1) pose est; (2) pose forecasting; (3) collision avoidance. We do 2 and 3. we discuss 2 in the next subsection. Maybe we should also discuss 3, as it's a main proposition.}

\smallskip
\myparagraph{Datasets for pose forecasting}
%\subsection{Datasets for pose forecasting}
%\MC{aggiungere questione delle collisioni + coesistenza robot, aggiungere InHard - Francesco} 
Human pose forecasting datasets cover a wide spectra of scenarios, see  Table~\ref{tab:symbiotic_h36_comparative}. 
Human3.6M~\cite{h36m_pami} covers a set of everyday scenarios, with actions like conversing, eating, greeting and smoking. Data were acquired using a 3D marker-based motion capture system, composed by 10 high-speed infrared cameras. AMASS~\cite{AMASS:ICCV:2019} is a collection of 15 datasets where daily actions were captured by an optical marker-based motion capture. Human3.6M and AMASS are standard benchmarks for human pose forecasting, with some overlap in the type of actions they deal with. The 3DPW dataset~\cite{vonMarcard2018} focuses on actions in outdoor scenarios, captured with a moving camera and 17 Inertial Measurement Units (IMU), embedded on a special suit for motion capturing~\cite{Corrales2011}. The recent  Multi-Person Extreme Motion Prediction with Cross-Interaction Attention  (ExPI)~\cite{guo2021multi} contains 16 different dance actions performed by professional dancers, for a total of 115 sequences, and is  aimed at motion prediction. ExPI has been acquired with 68 synchronised and calibrated color cameras and a motion capture system with 20 mocap cameras. Finally, the CHI3D and FlickrCI3D datasets~\cite{fieraru2020three} report 3D data taken from MOCAP systems to study human interactions.

%Obviously, it does not fit our aim, \emph{i.e.}, to present a realistic industrial setup where few low-cost cameras can reliably monitor HRC.

None of these datasets answer our research needs, i.e., a benchmark taken by a sparing, energy-efficient markerless system, focused on an industrial scenario (specifically HRC), where forecasting may be really useful for anticipate collisions between humans and robots.
Indeed, the only dataset related to industrial applications is InHARD~\cite{Dallel2020}. In this dataset humans are asked to perform an assembly task while wearing inertial sensors on each limb. The dataset is designed for human action recognition, and involves 16 individuals performing 13 different actions each, for a total of 4800 action samples over more than 2 million frames. Despite showcasing a collaborative robot, in this dataset the robot is mostly static, making it unsuitable for collision forecasting. Moreover, the use of inertial sensors is not representative of a real industrial use case.


%\subsection{Human Robot Collaboration}





==> src/Backup/bg_bk_2022-03-07.tex <==

%\subsection{Human pose forecasting}
\smallskip
\myparagraph{Human pose forecasting.}
Human pose forecasting is a recent field which has some intersection with human action anticipation in computer vision~\cite{li20} and HRC~\cite{duarte2018action}. Previous studies exploited Temporal Convolutional Networks (TCNs)~\cite{pavllo19,Bai18TCN,Gehring17,Li18} and Recurrent Neural Networks (RNNs)~\cite{fragkiadaki15,jain16,anand19}. Both architectures are naturally suited to model the temporal dimension.
%, in particular RNNs, even though TCNs have been reported to be sable than RNNs.
Recent studies have expanded the range of available methods by using Variational Auto-Encoders~\cite{Btepage2017AnticipatingMF}, specific and model-agnostic layers that implicitly model the spatial structure of the human skeleton~\cite{Aksan_2019_ICCV}, or Transformer Networks~\cite{Cai20}.

%\textbf{Pose forecasting using Graph Convolutional Networks (GCN)}
\smallskip
\myparagraph{Pose forecasting using Graph Convolutional Networks (GCN).}
Most recent research uses GCNs~\cite{Zhao20,stsgcn,li21,Dang21,Mao20DCT}.
In \cite{Mao20DCT}, the authors  have mixed GCN for modelling the joint-joint interaction with Transformer Networks for the temporal patterns. Others~\cite{Zhao20,stsgcn,li21} have adopted GCNs to model the space-time body kinematics, devising, in the case of~\cite{Dang21}, hierarchical architectures to model coarse-to-fine body dynamics.\\
We identify three main research directions for improving efficiency in GCNs:
%\textbf{ii}\ 
\textbf{i.}~space-time separable GCNs~\cite{stsgcn}, which factorizes the spatial joint-joint and temporal patterns of the adjacency matrix;
%\textbf{i}\
\textbf{ii.}~depth-wise separable graph convolutions~\cite{lai18}, which has been explored by~\cite{balcilar20} in the spectral domain;
and 
%\textbf{iii}\ 
\textbf{iii.}~sparse GCNs~\cite{shi21}, which iteratively prunes the terms of the adjacency matrix of a GCN.
Notably, all three techniques also yield better performance than the plain GCN.
Here, for the first, we bring together these three aspects into an end-to-end space-time-depthwise-separable and sparse GCN. The three techniques are complementary to improve both efficiency and performance, but their integration requires some structural changes (\emph{e.g.},\ adopting teacher-student architectures for sparsifying), as we describe in Sec.~\ref{sec:methodology}.

\smallskip
\myparagraph{Human Robot Collaboration (HRC). \MC{FABIO}}
%\FG{From how it reads, it seems pose estimation and collision avoidance are indeed THE tasks to address, which makes sense. So worth saying, at the very first line, "these are the tasks which matter most now, but no dataset is available". However, apart from this sentence (which actually relates to Sec 2.3), this subsection needs to spell out how we relate to HRC, which is currently missing.}\MC{CHecked, going to solve by shuffling the ordering of the subsections, rewriting some parts.}\\
HRC is the study of collaborative processes where human and robot agents work together to achieve shared goals~\cite{bauer2008human,castro2021trends}. Computer vision studies on HRC are mostly related to pose estimation ~\cite{OpenPoseTPAMI19,Lemmerz2019,Garcia-Esteban2021} to locate the articulated human body in the scene; head pose estimation~\cite{patacchiola2017head} and gesture recognition~\cite{liu2018gesture} are used to facilitate the communication with the robot.
%Sarafianos2016,
%Tan2010,
%Beckert2018,
%Araiza-Lllan2018,
%and motion planning with collision avoidance~\cite{Chen2018,Kanazawa2019,Nascimento2020,Kang2019,Costanzo2020}
%Beltran2018,Lim2021}. 
%Other relevant tasks are head pose estimation~\cite{patacchiola2017head} and gesture recognition~\cite{liu2018gesture}. Relating to pose estimation, we highlight ~\cite{Tan2010,Beckert2018,Araiza-Lllan2018,Lemmerz2019}, where pose estimation approaches are specifically designed to monitor HR collaboration \FG{not clear this part. do you mean "safety"? Also do not use HR, preferable HRC.}. 
In~\cite{Chen2018,Kanazawa2019,Nascimento2020}, methodologies for robot motion planning and collision avoidance are proposed; their study perspective is opposite to ours, since we focus on the human operator. In this regard, the works of~\cite{Beltran2018,Kang2019,Costanzo2020,Lim2021} model the operators' whereabouts through detection algorithms which approximate human shapes using simple bounding boxes. 
Approaches that predict the human motion during collaborative tasks are in~\cite{torkar2019rnn,zhang2020recurrent} using RNNs and in~\cite{vianello2021human} using Guassian processes. In~\cite{laplaza2021attention}, the robot end-effector position is modelled too, considering some handover interactions.  As motion prediction engine,  DCT-RNN-GCN~\cite{Mao20DCT} is considered, against which we compare in the experiments. 
Notably, in all of the above-cited cases, no datasets have been provided, while this paper provides \dataname{}. Additionally, we are the first to have considered and predicted collisions in an HRC context, for a set of industrial actions.   

%Notably, we are the first in proposing human pose forecasting in a HRC context,  \emph{providing the first dataset taken in an industrial setup, equipped with HR collisions}, plus associated baselines, to promote further research.
%\FG{emphasize common and distinct aspects, distinguishing: (1) pose est; (2) pose forecasting; (3) collision avoidance. We do 2 and 3. we discuss 2 in the next subsection. Maybe we should also discuss 3, as it's a main proposition.}

\smallskip
\myparagraph{Datasets for pose forecasting.}
\input{tab/CHICO_comparative_BAK} \label{sec:cohre_dataset}
%\input{tab/symbiotic_h36_comparative} \label{sec:cohre_dataset}
%\subsection{Datasets for pose forecasting}
%\MC{aggiungere questione delle collisioni + coesistenza robot, aggiungere InHard - Francesco} 
Human pose forecasting datasets cover a wide spectrum of scenarios, see  Table~\ref{tab:symbiotic_h36_comparative} for a comparative analysis. 
%
Human3.6M~\cite{h36m_pami} covers a set of everyday scenarios, with actions such as conversing, eating, greeting and smoking. Data were acquired using a 3D marker-based motion capture system, composed of 10 high-speed infrared cameras. AMASS~\cite{AMASS:ICCV:2019} is a collection of 15 datasets where daily actions were captured by an optical marker-based motion capture. Human3.6M and AMASS are standard benchmarks for human pose forecasting, with some overlap in the type of actions they deal with. The 3DPW dataset~\cite{vonMarcard2018} focuses on actions in outdoor scenarios, captured with a moving camera and 17 Inertial Measurement Units (IMU), embedded on a special suit for motion capturing~\cite{Corrales2011}. The recent ExPI dataset~\cite{guo2021multi} contains 16 different dance actions performed by professional dancers, for a total of 115 sequences, and is  aimed at motion prediction. ExPI has been acquired with 68 synchronised and calibrated color cameras and a motion capture system with 20 mocap cameras. Finally, the CHI3D dataset~\cite{fieraru2020three} reports 3D data taken from MOCAP systems to study human interactions.

%Obviously, it does not fit our aim, \emph{i.e.}, to present a realistic industrial setup where few low-cost cameras can reliably monitor HRC.

None of these datasets answer our research needs, i.e., a benchmark taken by a sparing, energy-efficient markerless system, focused on an industrial scenario (specifically HRC), where forecasting may be really useful for anticipating collisions between humans and robots.
Indeed, the only dataset related to industrial applications is InHARD~\cite{Dallel2020}. In such dataset humans are asked to perform an assembly task while wearing inertial sensors on each limb. The dataset is designed for human action recognition, and involves 16 individuals performing 13 different actions each, for a total of 4800 action samples over more than 2 million frames. Despite showcasing a collaborative robot, in this dataset the robot is mostly static, making it unsuitable for collision forecasting. Moreover, the use of inertial sensors is not representative of a real industrial use case.


%\subsection{Human Robot Collaboration}





==> src/Backup/concl_bk_2022-03-07.tex <==

We have considered HRC and the case of human collaboration with a robotic arm in a real industrial assembly line.
HRC requires the accurate anticipation of human motion, for which we have proposed SeS-GCN pose forecasting model, a new all-separable and sparse GCN which improves prediction accuracy (3.6\% less error than SoA) and efficiency (14.5\% less parameters).
To benchmark HRC, we have also proposed the first dataset \dataname of pose trajectories in a real industrial assembly line. \dataname is fine-grained, featuring nuanced motions for difference actions, and challenging.
The performance of SeS-GCN (average error of 57.3mm at 1.6sec) sets a positive milestone, but \dataname will likely foster further future progress.
% We have proposed a modern Separable Sparse Graph Convolutional Network (SeS-GCN) for human pose forecasting and Symbiotic:Human, an innovative human-robot collaboration dataset, the first of its kind.
% Our technique has produced a smaller error in millimetres than the state-of-the-art, requiring less parameters. Such efficiency and accuracy is essential in an environment where humans and cobots collaborate, in order to avoid collisions.\\
% By providing an industrial dataset acquired in a real-world scenario, this work hopes to open up future research aimed at human-robot coexistence in a shared ecosystem.


==> src/Backup/exp_res_bk_2022-03-06.tex <==

%Our all-Separable model benefits from the few robust connections between its nodes, which are encoded with group convolution. The techniques involved have a positive impact on limiting the number of parameters, increasing the efficiency of the model and improving performance. We illustrate the sensitivity of the model to each of these methodologies and show their impact numerically.

%First 
We benchmark the proposed SeS-GCN model on the large and established Human3.6M~\cite{h36m_pami}. In Sec.~\ref{subsec:model_choices}, We analyze the design choices corresponding to the models discussed in Sec.~\ref{sec:methodology}. Then we compare with the state-of-the-art in Sec.~\ref{subsec:comparison_h36m}. SeS-GCN outperforms competing techniques, while requiring same memory and run time.



\medskip
\myparagraph{Human3.6M} \cite{h36m_pami} is an established dataset for pose forecasting, consisting of 15 daily life actions (e.g. Walking, Eating, Sitting Down) recorded for 7 actors. From the original skeleton of 32 joints, 22 are sampled as the task, representing the body kinematics. A total of 3.6 million poses are captured at 25 fps. In line with the literature~\cite{Mao20DCT,Julieta17}, subjects 1, 6, 7, 8, 9 are used for for training, subject 11 for validation, and subject 5 for testing.

\input{tab/model_construction_ALTERNATIVE}

\medskip
\myparagraph{Metric.} \label{par:metrics} The prediction error is quantified via the MPJPE error metric~\cite{h36m_pami,Mao19LTD}, which considers the displacement of the predicted 3D coordinates \textit{wrt} the ground truth, in millimeters:
\begin{equation}
L_{\text{MPJPE}}= \frac{1}{VK} \sum_{k=T+1}^{T+K} \sum_{v=1}^{V} ||\hat{\boldsymbol{x}}_{vk}-\boldsymbol{x}_{vk} ||_{2}
\end{equation}




\subsection{Modelling choices of SeS-GCN}
\label{subsec:model_choices}
We review and quantify the impact of the modelling choices of SeS-GCN:



\medskip
%\myparagraph{Space-time factorization: GCN Vs.\ STS-GCN}
%\fab{we start off with the current best, sts-gcn. priviledged tim-time and joint-joint.}
%\fab{Refer to the table, comparison with gcn.}
%STS-GCN~\cite{stsgcn} has empirically demonstrated that both the performance and the efficiency of a vanilla GCN are improved when privileging the graph connections corresponding to time-time and joint-joint, via factoring the graph adjacency matrix. In Table~\ref{tab:ablation}, we validate the findings and reproduce their results, obtaining an error of 75.6mm at a 1 sec forecasting horizon while only requiring 57.6k parameters.
\myparagraph{GCN approaches.} Table \ref{tab:ablation} empirically demonstrates the different approaches adopted in the literature that improve the performance of a vanilla GCN. Specifically, the best improvement in both performance and efficiency corresponds to the technique that factorizes the graph adjacency matrix \cite{stsgcn}. It should be noted that DW-GCN \cite{lai18}  increases the performance of a vanilla GCN by 3.4\% despite having the same number of parameters. This efficiency allows the construction of deeper models, while keeping the accuracy of the network itself high.




%\input{tab/symb_quantitative_full}

\smallskip
\myparagraph{Deeper (depthwise) networks.} % deeper STS-GCN Vs.\ STS-GCN+MLP}
It is a long standing belief that Deep Neural Networks (DNN) owe their performance to depth~\cite{zeilerfergus,vgg,resnet,resnext}. However, deeper models require more parameters and have a longer processing time. Seeking both better accuracy and efficiency, we consider three main directions:
(1) add GCN layers; (2) add MLP layers with shared parameters at each node, between layers of GCNs; (3) add MLP layers with shared parameters which leverage depthwise separable convolutions.

As shown in Table \ref{tab:ablation}, deeper STS-GCN models with more layers (we have tested 5 and 6) boost accuracy by just 0.7\% (errors go from 75.6 to 75.1 mm in the case of 5 layers), by adopting only 68.6k parameters. 
%This is somehow surprising, because the model is still relatively shallow, compared to deep convolutional works~\cite{Szegedy15}.
%This may be due to over-smoothing, as also maintained in \cite{Oono20, huang2021, li2018deeper} 
%\fab{more ref to oversmoothing?}
%, i.e. deeper GCNs have larger receptive fields for their nodes, which make the nodes indistinguishable, at from the graph perspective.
This increase in performance due to an increase in network depth paves the way for the inclusion of extra MLP layers with shared parameters at the graph nodes (STS-GCN w/ MLP). Nevertheless, this approach decreases performance and increases the number of parameters. 
%This finding has been explained as over-smoothing since the nodes of a deeper GCN have larger receptive fields and become indistinguishable.~\cite{Oono20}.

%Following the second direction and adding extra MLP layers with shared parameters at the graph nodes also decreases or leaves performance unaltered, but it increases the number of parameters.
By contrast, adopting extra MLP layers based on depthwise-separable convolutions results in a reduced error of 73.6mm, which is already beyond the state-of-the-art, at a very minor increase of the parameter count, from 57.6k to 70.0k. This improvement may be explained as the positive effect of limiting cross-channel talks within the GCN layer computation of Eq.\eqref{eq:allsep1}, which parallels similar arguments from the literature of convolutional networks~\cite{chollet17, howard17}


%A grouped convolution placed within the GCN to allow the model to get an equivalent mapping for each feature in the graph, necessitating the inclusion of an MLP to establish a connection between them. Depthwise convolution does not contribute directly to the efficiency of the model, leaving the number of learnable parameters almost unchanged. The impact is clear looking at the MPJPE error, by adopting matrix factorization and this technique the model performance is improved by 2.3\% \textit{wrt} the current state-of-the-art.\\
%By adopting depthwise convolution it is permissible to map features in high dimensionality, however FigX, blue line, shows that performance remains invariant, FigX xxx line as the multiplication factor increases. It is therefore preferable to keep the dimensionality low in order to be efficient.




\medskip
\myparagraph{Sparsifying GCNs and the proposed SeS-GCN.}
Finally, we target efficiency by model compression.
Trends have reduced the size of models by reducing the parameter precision~\cite{rastegari2016xnornet}, by pruning and sparsifying some of the parameters~\cite{molchanov2017pruning}, or by constructing teacher-student frameworks, whereby a smaller student model is paired with a larger teacher to reach its same performance~\cite{hinton2015distilling,muyang20}. Note that the latter is currently a trend in deploying very large networks such as Transformers~\cite{benesova2021costeffective}.

We start off by compressing the model with sparse adjacency matrices~\cite{shi21}. Sparse-GCN~\cite{shi21} proposes to do so by iteratively optimizing the learnt parameters and the masks to select some.
As illustrated in Table~\ref{tab:ablation}, this does not make a viable direction, since the increase in parameters almost 74\% corresponds to a much larger error, up to 74.8mm, \textit{wrt} STS-DW-GCN.

Reminiscent of teacher-student models, in the proposed SeS-GCN we first train a teacher GCN, then use its learnt parameters to sparsify the affinity matrices of a student GCN, which is then trained from scratch. Compared to Sparse-GCN~\cite{shi21}, the reduction in the number of parameters is more significant (53.2\%) and the final forecasting error is further reduced to 72.9mm, our current best.


%Recently, SGCN \cite{shi21} has been proposed as the first GCN with sparse adjacency matrices. The mechanism that allows them to sparsify is adaptively built on the input, and the masks are learned end-to-end during training. Another possible approach is having two successive generations of models in a teacher-student fashion. In this case, the student model leverages a mask determined by the adjacency matrix of the previously trained teacher model. The mask is thus fixed during the student network training and allows one to learn only a smaller number of connections, the most promising ones to reconstruct the human motion. From Table \ref{tab:model_table} it is possible to compare the two modes of sparsification: while the end-to-end network allows a saving of more than 40\% on the number of parameters compared to the non-sparse version, it worsens performance. On the other hand, the teacher-student strategy still allows a saving, just 84.4\% of the parameters are saved \textit{wrt} the non-sparse version. At the same time, the performance grows considerably, reaching a total MPJPE of 72.9mm and setting a new best on state-of-the-art.


%\fab{please redo this section. Need to start from saying that "Most recently, SGCN has been proposed as the first GCN with sparse adjacency matrices"... then say that sgcn is end-to-end, and that another plausible approach is the teacher-student, whereby the students leverage the sparsity as determined by a teacher model, previously trained.}
%\fab{Ideally, certain graph connections in the body kinematics are key to uncerstanding the motion. Priviledging those results in better performance. In any case in a GCN nodes may be reached with multiple hops. This also corresponds to a less complex model, so less prone to overfitting. See Table, sparsity can be obtained via the following: (1) end-to-end sts+dw+sparse; (2) teacher-student sts-dw-sparse. (1) adopt [ref], since it is end to end, then it effectively adds at training the masking parameters. Overall it's improving efficiency but descreasing in performance, which is not desirable. (2) learns a sts-dw, then uses its A's to sparsify the body kinematics connections. Then the student model can be trained from scratch leveraging the teacher's mask. We additionally test an iterative approach, where the teacher is directly sparsified and the model fine-tuned.}

%It is feasible that not all the parameters of the space-time matrix are needed to capture the movements of the human body, by applying a mask derived from the matrix itself, the parameters can be decreased, leaving only the strongest connections on. The framework thus implemented has a large impact on the capacity of the graph, decreasing the parameters by 40.2\% in an end-to-end all-Separable model wrt current best technique. However, performance declines, making this framework non-preferable for human-robot collaboration.\\ The sparsification technique can then be considered differently. Let our proposed SeS-GCN model, last row in Table \ref{tab:model_table}, learn a mask of the space-time matrix that favours robust connections, then apply that mask to the same matrix from scratch. In our directed and signed graph, this methodology allows us to focus on those connections, positive or negative, that are established between nodes. SeS-GCN achieves a performance increase on Human3.6M \cite{h36m_pami} of 3.6\% in the longest prediction and uses 14.5\% less parameters than the state-of-the-art \cite{stsgcn}.  \\
%The model is able to match the current best technique by having one third of the parameters. FigX xxx line shows how the model's performance decreases as the cutoff increases, with a cutoff of 0.3 only 8\% of the space-time connections are taken into account.\\
%SeS-GCN reaches its peak by thresholding the space-time matrix at the end of the training. Leaving the model free to learn the correlations among the nodes it is possible to execute the cut of the connections a posteriori, favouring the strongest ones. The learnt mask is inserted as a constant in the same model, letting now the model focus on the connections left on. The xxx line in FigX represents a sensitivity analysis of the model, which achieves the best performance with a thresholding at 0.3. SeS-GCN achieves a performance increase of 3.6\% over the current state of the art, using 14.5\% less parameters.



\subsection{Comparison with the state-of-the-art}
\label{subsec:comparison_h36m}
In Table \ref{tab:h36m_quantitative_full}, we evaluate the proposed SeS-GCN against three most recent techniques, over a short time horizon (10 frames, 400 msec) and a long time horizon (25 frames, 1000 msec). The first,
%The comparison, shown in Table \ref{tab:h36m_quantitative_full}, is \textit{wrt} state-of-the-art models such as 
DCT-RNN-GCN~\cite{Mao20DCT}, uses DCT encoding, then motion attention and RNNs. The other two, MSRGCN~\cite{Dang21} and STS-GCN~\cite{stsgcn} adopt GCN-only frameworks, the second being the current best pose forecasting approach.\\
\myparagraph{Short-term prediction.} At the prediction horizon of 400 milliseconds, the proposed model outperforms the state-of-the-art in each action considered. The largest margin occurs in complex actions such as Sitting and Directions, where there is a performance improvement of up to 5.8\%. SeS-GCN gives an average improvement of 2.7\% \textit{wrt} the current best technique in a 10-frame prediction.\\
\myparagraph{Long-term prediction.} Table \ref{tab:h36m_quantitative_full} presents a comparison on a prediction time of 1 second (25 frames). The increase in performance ranges up to 6.9\%, even for static actions such as Eating, Taking Photo and Waiting. Across all actions, SeS-GCN decreases the current best prediction error by 3.6\%.

\input{tab/h36m_quantitative_full}

==> src/Backup/exp_res_sd_2022-03-07.tex <==


%\paragraph{\dataname} %The 8 industrial actions have the human pose captured by with 17 joints at a framerate of 20 fps. 
Similarly to the protocol adopted with Human3.6M, to train the pose forecasting approaches we used two subjects for validation (2,10), two subjects for testing (1,20) and the remaining 16 subjects for training. We use MPJPE as training and testing loss (see Sec.~\ref{par:metrics}).%\MC{forse con 20 soggetti previsti, fare un singolo LOO non ha molto senso... meglio tenere 8-10 soggetti? Uniformare con 2 soggetti di test}
 It is worth noting that training was performed on the sequences without collisions, since we are interested in modeling the ``correct'' collaborative human behavior, and not the human retractions and the pauses due to the collisions. In fact, after the collision, the robot stops for 2 seconds, during which the human operator usually stand still, waiting for the robot resuming its activity. 
%\FG{Update test id and mention collisions}

\subsection{Pose forecasting experiments}
\label{subsec:quantitative_symb}


\input{tab/CHICO_quantitative_full}

As shown in Table \ref{tab:CHICOresults} SeS-GCN outperforms on average the current state-of-the-art \cite{stsgcn} on \dataname dataset. Since the acquisition is performed at 20 frames-per-second, the short-range (10 frames) coincides with a prediction time of 500 milliseconds while the long-range (25 frames) correspond to 1250 milliseconds. This timing is sufficient to capture a representative portion of the action
%encapsulates an action that 
the operator performs in a collaborative environment. Notably, the prediction horizon is longer than Human 3.6M due to the lower framerate, and is longer in general than all of the pose forecasts in the literature.



% \begin{figure}[t!]
%     \centering
%     \includegraphics[page=3,width=0.99\linewidth]{fig/CVPR_one_col_figures.pdf}
%     \caption{Example of two actions taken from our proposed \dataname dataset: (a) Lift, (b) Polish. See details in Sec. \ref{subsec:actions}.
%     }
%     \label{fig:actions}
%     \vspace{-0.5cm}
% \end{figure}

%\medskip
\myparagraph{Short-term prediction.} 
In this setting the model shows an error of 28.7mm on average and exceeds the performance of the other baselines on all the two-handed actions. The network performs 21.8\% better than the current state-of-the-art \cite{stsgcn} and outperforms MSR-GCN \cite{Dang21} and DCT-RNN-GCN \cite{Mao20DCT} by at least 30.6\%.
% DRAFT TO REMOVE SEC.7 - LIMITATION
%Despite the excellent performance exhibited by our model, we are aware that some specific actions (e.g. high-speed grasping) would require greater precision in localizing and forecasting human joints in order to establish a safe and consistent collaboration with a robot.



%\medskip
\myparagraph{Long-term prediction.} 
It is easy to see that, on a time horizon of 1250 milliseconds, which is more than twice the short-term range,  the error was in average less than double on average. This is obviously determined by the type of the actions, which take place on a restricted space. Anyway, this indicates that the SeS-GCN captured the repetitive nature of the actions.

%Compared to the other approaches, the error difference is not so significant when it comes to actions which take place on a restricted space (e.g. Span heavy, Polish).
In the most complex actions (e.g. \emph{Low Lift}, \emph{Polishing}), where the operator motion is larger, SeS-GCN achieves up to 15.9\% performance increase compared with the second best technique. 
%\AS{da ricontrollare le 4 righe qui sopra, nomi azioni e numeri sembrano errati}

For a sanity check of results, we have also evaluated the performance of a trivial zero velocity model. \cite{Julieta17} has found that keeping the last observed positions may be a surprisingly strong (trivial) baseline. For CHICO, the zero velocity model scores an MPJPE of 116.1 mm at 25-frames, which is $>$2x worse than the 53.0 mm score of SeS-GCN. This is in line with the large-scale dataset Human3.6M~\cite{h36m_pami}, where the performance of the trivial model is 153.3 mm, also $>$2x worse than the score 72.9 mm of SeS-GCN.

%Results  in Table \ref{tab:quantitative_symbiotic} show that our model is able to forecast the movement of arms and wrists with a minor number of parameters. 
%As shown in \ref{tab:model_table}, SeS-GCN has on average 2.4\% lower error compared to the second best approach \cite{stsgcn}.

%\label{subsec:qualitative_eval}
%\subsection{Qualitative evaluation}
%\label{subsec:qualitative}

%In Fig.~\ref{fig:qualitative_CoHRE} we show some qualitative results. Coherently with Table~\ref{tab:quantitative_symbiotic}, SeS-GCN provides excellent predictions for poses from actions such as Lift or Place objects. Our model preserves movement during the course of the action, and does not differ from ground truth (in red).
\begin{figure}[t]
    \centering
    % \includegraphics[page=4,width=0.5\linewidth]{fig/CVPR_one_col_figures.pdf}
    \includegraphics[width=0.5\linewidth]{fig/joint_errors.png}
    \caption{Average MPJPE distribution for all actions in \dataname on different 17 joints for (a) short-term (0.5 s) and (b) long-term (1.25 s) predictions. The radius of the blob gives the spatial error with the same scale of the skeleton. \MC{check, double blobs, nose is missing say it is simplified}}
    \label{fig:error}
   \vspace{-0.5cm}
\end{figure}
Fig.~\ref{fig:error} shows a distribution of the error per joint calculated over all the actions, for the horizons 0.5s and 1.25s. In both the cases the error is larger as soon  as we consider nodes that are more towards the extremes of the skeleton, since they are the ones that move the most.

%there is a lower error for the upper limbs than for the legs. The reason is due to the acquisition setup: actually, legs have been captured by a single acquisition device and this brought to a noisier signal. On the upper limbs, the elbows showed a slightly higher error than the hand (except the longer time horizon, left arm). This is because the detection of the elbow was more difficult to perform by the pose estimator, so that even in this case the reason is due to the acquisition phase, and not to the forecasting model.

\subsection{Collision detection experiments}
Here we evaluate the ability of  anticipating the collisions with the robotic arm. We assume to know the future trajectory of the cobot, since we scripted its movement routine beforehand. %the robot can deviate from the routine only in the case of collisions, in which case it stops, resuming the movement after 2 seconds, from where it had stopped. This stop-and-go is the standard behaviour of cobots in case of collisions~\cite{mikhel2018collision} and can be understood as an iteration of reinforcement learning, in which the robot hypothesizes its possible future, deriving a reward based on the prediction of the movement of the human operator~\cite{bai2015intention,choi2022preemptive}. However, it is important to note that decision-making for motion planning is not the focus of this paper and will be considered in a subsequent work.  

In rough words, we individuate a collision whenever the future trajectory of the human will bring him/her closer than a safety distance threshold. Formally, given a test sequence reporting a specific action (see for example Fig.~\ref{fig:teaser} for \emph{Lightweight pick and place}), we analize it by a 500 msec. observation window, with a stride of 500 msec, predicting the following 1250 msec.

 %. We do not consider the 500msec shorter prediction horizons, \MC{since it is too short to allow a proper reaction... su questa frase ci si gioca il paper!} \MC{occhio se si fa vedere il grafico temporale} 
A collision is predicted at a given prediction window when the \emph{minimal HR-distance} of the operator is lower than  $\tau_{prox}=5cm$, at least for a single frame. As minimal HR-distance we mean the minimum euclidean distance between each stick of the human skeleton and the cobot. 
As technicality, all the limbs of robots and humans are approximated by cylinders~\cite{minelli2020iros}, whose diameter in the case of the robot is fixed at 8cm, and the diameter of the body sticks are predefined, taken by a human atlas\footnote{This model is rough, and can be ameliorated by considering parametric models as SMPLE [ref] which will be considered for a future work.} The $\tau_{prox}$ threshold is the net distance between the border of the cylinder of the robot, and the border of the specific limb. 
%In Fig.~\ref{fig:collision_sig}
%\MC{Abbiamo specificato quali sono le policy di pose forecasting che hanon portato ai res della Tab.4? Con che passo vengono spezzettate le singole sequenze lunghe 500 e 1250? Esiste un overlap?}



%which we infer, will bring him/her closer than a safety distance threshold $\tau_{prox}$. This comes from the recent literature about collision avoidance in robotic setups~\cite{minelli2020iros} where all the limbs of robots and humans are approximated by cylinders. 
%Since the inference step requires XXX seconds, which amounts to $T_{comp}$ frames, we simulate a real system by considering a prediction which is $K-T_{comp}$ frames ahead.
%
%In Fig.~\ref{fig:roc_collision} we report the ROC curves for all the prediction methods. We can appreciate how the proposed \gcnname is the best performing. 
%We also set $\tau_{prox}=XXcm$ and 
We compute precision, recall and F$_1$ scores, reported in Table~\ref{tab:collisions}. Here it is possoble to note that...\MC{completare}. %It is interesting to see that longer horizon predictions, despite are less precise, give better score.        

% To predict whether there will be a collision between human and robot in the forecasting horizon we adapted an approach proposed in~\cite{minelli2020iros}. We model both the agents as a composition of capsules, that enclose each limb into the fittest and simplest shape. \FG{Capsules may be confused with capsuleNet. Also probably best to directly argue for the specific shapes, cylinders?}
% Given  a  pair  of  Cartesian  points,  a  capsule  is  an object composed by two hemispheres, centered in that points, and a cylinder, with longitudinal axis linking the two points.
% \MC{Francesco, spostare a 6.2} \FG{If you move it to 6.2 (totally agreed from my side) try to simplify the method (that they don't complain about not including the section into the model part). Eg skip the hemispheres, remove the "capsule", just say each limb is approximated by a cylinder, so it can generate a collision. Say how the radius is chosen.}




\begin{table}[ht]
  \begin{minipage}[b]{.55\linewidth}
      \centering
      \resizebox{\linewidth}{!}{
        \begin{tabular}{|l|c|c|c||c|}
          \cline{1-4}
          \textit{Time Horizon (msec)} & \multicolumn{3}{c||}{ \textbf{\textit{1250}}} \\ \hline
          Metrics &  \textit{Prec} & \textit{Recall} & \textit{F}$_1$ & \textit{Inference Time} \\ \hline
          \multicolumn{1}{|c|}{DCT-RNN-GCN~\cite{Mao20DCT}}&  &  & &  $9.1 \times 10^{-3}$\\
          \multicolumn{1}{|c|}{MSRGCN~\cite{Dang21}}&  &  &  & $25.2 \times 10^{-3}$\\
          \multicolumn{1}{|c|}{STS-GCN~\cite{stsgcn}}& 0.81 & 0.69 & 0.74 & $2.3 \times 10^{-3}$ \\ \hline
          \multicolumn{1}{|c|}{Ours} & 0.86 & 0.64 & 0.73 & $2.3 \times 10^{-3}$\\ \hline
        \end{tabular}
      }
    \caption{Collision detection performances \MC{motivare l'orizzonte lungo}}
    \label{tab:collisions}  
  \end{minipage}\hfill
\begin{minipage}[b]{0.435\linewidth}
\centering
\includegraphics[width=60mm]{fig/Collision_detection.jpeg}
\captionof{figure}{Temporal analysis of a collision, in a frames VS distance space, where the distance is computed between the wrist and the hand effector joints}
\label{fig:collision_sig}
\end{minipage}
\end{table}
% \begin{table*}[!htb]
% \centering
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{c|cc|cc|c|}
% \cline{2-6}
%                                     & \multicolumn{2}{c|}{precision}        & \multicolumn{2}{c|}{recall}    & Inference Time (sec)   \\ \cline{1-5}
% \multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{17 Joints}} \\ \hline
% \multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 39.3               & 57.9                & 16.9               & \textbf{26.9}    &     $9.1 \times 10^{-3}$              \\
% \multicolumn{1}{|c|}{MSRGCN \cite{Dang21}}       & \textbf{26.8}      & \textbf{47.5}       & 17.0               & 31.4                &      $25.2 \times 10^{-3}$         \\

% \multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & 30.6               & 61.9                & 16.0               & 33.3         &     $2.3 \times 10^{-3}$       \\ \hline
% \multicolumn{1}{|c|}{Ours}          & 30.4               & 59.6                & \textbf{15.3}      & 31.0   &    $2.3 \times 10^{-3}$     \\ \hline
% \end{tabular}}
% \caption{Collison detection perfomances}
% \label{tab:collisions}
% \end{table*}
%The most part of the actions in \dataname have been performed with the upper-body and this is mostly reflected by the prediction's accuracy on the arms keypoints that is higher than the rest of the body. From the HRC point of view, it is mandatory having high prediction accuracy especially for the portion of the body coexisting with the robot.
%From this perspective the model learns effectively the movements of the human.


% \begin{figure}
%     \centering
%     \includegraphics[width=.4\textwidth]{fig/roc_collisions.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% left out, not delete please
%\paragraph{Implementation details} The proposed model consists of an encoder and a decoder.
%Four SepGCN layers compose the encoding part of the graph that maps from 3D x,y,z coordinates to new 3D values, learning the connections between them. At each step a batch normalization \cite{batchnorm15} is performed and residual connections are adopted.
%The model is developed in Pytorch and its optimiser is ADAM \cite{adam15}. 
%On Human3.6M the training takes place for 40 epochs, we set the batch size to 256, the learning rate to 0.01 and milestones that adopt a decay rate of 0.1 at epochs 25, 30 and 37.
%On an NVIDIA RTX 2060 GPU the learning process takes 30 minutes, while evaluation for a batch size 8 takes 0.006 seconds.


==> src/Backup/intro_bk_2022-03-05.tex <==
\begin{figure}[ht]
\begin{subfigure}{\linewidth}
  \centering
  % include first image
   \includegraphics[page=8,width=0.8\linewidth]{fig/CVPR_one_col_figures.pdf}  
  \caption{Lifting}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{\linewidth}
  \centering
  % include second image
   \includegraphics[page=9,width=0.8\linewidth]{fig/CVPR_one_col_figures.pdf}  
  \caption{Heavyweight pick and place}
  \label{fig:sub-second}
\end{subfigure}
\caption{Qualitative results for long-term predictions on two actions from our proposed \dataname{} dataset. One every four frames are shown. Red/black identifies prediction/ground truth. Note that our proposed model correctly predicts the pose. See Sec.~\ref{subsec:qualitative} for a discussion.}
\label{fig:qualitative_CoHRE}
\vspace{-0.5cm}
\end{figure}

Collaborative robots (cobots) and modern Human Robot Collaboration (HRC) depart from the traditional separation of functions of industrial robots~\cite{Stein2020}, since cobots share the same workspace as the human workers~\cite{iso15066}. Additionally cobots and humans perform actions concurrently and they will therefore physically engage in contact. While there is a clear advantage in increased productivity~\cite{Rodriguez-Guerra2021} (improved by as much as 85\%~\cite{Shah2011}) due to the minimization of idle times, there are challenges in the workplace safety~\cite{Gualtieri2020}: it is not about whether there will be contact, but rather about understanding its consequences~\cite{Matthias2016}.



The pioneering work of Shah et al.~\cite{Shah2011} has already shown that, in order to seamlessly and efficiently interact with human co-workers, cobots would need to abide by two collaborative principles: \textbf{\emph{(i)}} Making decisions on-the-fly, and \textbf{\emph{(ii)}} Considering the consequences of their decision on their teammates. The first calls for promptly and accurately detecting the human motion in the workspace. The second principle implies that cobots need to anticipate pose trajectories of their human co-workers.



Motivated by these problems, the first contribution of our work is a novel Separable Sparse Graph Convolutional Neural Network model (\gcnname{}) for human pose forecasting. Pose forecasting requires understanding of the complex spatio-temporal joint dynamics of the human body and recent trends have highlighted the promises of modelling body kinematics within a single GCN framework~\cite{shi21,Dang21,stsgcn,li21,Wang_21,Zhao20,cui20,li20,Mao19LTD}.
We designed \gcnname{} with performance and efficiency in mind and we did so by bringing together, for the first time, three main modelling principles: separable graph adjacency matrices ~\cite{stsgcn}, sparse graph adjacency matrices~\cite{shi21}, and depthwise-separable convolutions~\cite{chollet17,howard17}. Our model is the first GCN to use a teacher-student sparsification framework and the first fully separable GCN in space, time and channels. \gcnname{} results in a lightweight and deep model, mindful of the over-smoothing~\cite{Oono20} problem, and is described in detail in Sec.~\ref{sec:methodology}.



%%MARCO:https://journals.sagepub.com/doi/abs/10.1177/02783649211050677?journalCode=ijra  dataset HR
This work also presents \dataname{}, the very first Human Robot Collaboration benchmark where safety plays a crucial role.
\FG{Need to include "industrial" too, one keyword in Fig 1.}
\dataname{} contains 3D pose and trajectories of XX human operators when collaborating within a shared workspace with a collaborative robotic arm \emph{KUKA LBR iiwa} on YY different actions, taken on a real industrial assembly line with a marker-less setup.
The recorded human actions are fine-grained (e.g.\ lifting objects from the ground and placing them on a table close to the cobot \FG{report a better example of fine grained, eg small-large range, clock-wise-anti-clockwise, or mention the reduced workspace?}) and therefore demand minimal trajectory forecasting error to be discerned \FG{but no activity recognition is pursued}.
The additional aim of \dataname{} is to bring safety in HRC at another level, in which collisions are not detected by mechanical events (trasmission of contact wrenches, control torques, sensitive skins), but foreseen by visual forecasting. In fact, mechanical events imply that the collision does happen; on the contrary, we want to predict it \emph{before} it happens. \FG{I can't be convinced on the argument on safety. These robots ARE safe, else we could not test them/ask anyone to record these experiments. However collisions are time-consuming, break concentration, and are anti-social (anti-colab), not sustainable in industry in the long term.}
%%MARCO https://d-nb.info/1211397823/34 
To this sake, \dataname{} contains ZZ genuine collisions generated by  consensual human operators collaborating on quick activities with the cobot choosing randomly its routines from one point to another \FG{randomly? maybe mention arbitrary decisions and multi-modality, eg humans have multiple pathways and start/stop moments to move things from A to B, even if the action is carefully scripted. In a h-cobot scenario the collision will occur, unless both parties watch out for the "intention" of the other}. Despite collisions are real, it is worth noting that they were harmless, since the cobot was setup to have maximum sensibility, and the actions were designed to have the right arm of the human operator potentially colliding with the robot. 
 
 
 
 %The data acquisition process, as well as ethical issues and limitations of \dataname{} are discussed in Sec.~\ref{sec:cohre_dataset}.




\gcnname{} is thoroughly tested on the well-known, large-scale pose forecasting dataset Human 3.6M~\cite{h36m_pami}, where it outperforms the current best technique~\cite{stsgcn}, reducing its error by 3.6\% on the longer-term future predictions at 1$s$, while having 14.5\% less parameters. Results are also encouraging on \dataname{}, where it yields an error of 57.3$mm$ (MPJPE) at 1.6$s$, with negligible runtime. Additionally, and for the first time in the literature, we have been able to measure the accuracy in predicting collisions with the robot, by checking whether the predicted trajectory of the human was colliding with the one of the robot. In particular, we obtain the XX of precision and YY of recall \FG{maybe adopt the F1-score for a balanced since metric?}



This provides the effective anticipation of the future which HRC demands. Experiments on both Human 3.6M and \dataname{} are described in detail in Secs.~\ref{sec:experimental_results_h36m} and~\ref{sec:experimental_results_sd} respectively.

==> src/Backup/intro_bk_2022-03-07.tex <==
%\begin{figure}[ht]
%\begin{subfigure}{\linewidth}
%  \centering
%  % include first image
%   \includegraphics[page=8,width=0.8\linewidth]{fig/CVPR_one_col_figures.pdf}  
%  \caption{Lifting}
%  \label{fig:sub-first}
%\end{subfigure}
%\begin{subfigure}{\linewidth}
%  \centering
%  % include second image
%   \includegraphics[page=9,width=0.8\linewidth]{fig/CVPR_one_col_figures.pdf}  
%  \caption{Heavyweight pick and place}
%  \label{fig:sub-second}
%\end{subfigure}
%\caption{Qualitative results for long-term predictions on two actions from our proposed \dataname{} dataset. One every four frames are shown. Red/black identifies prediction/ground truth. Note that our proposed model correctly predicts the pose. See Sec.~\ref{subsec:qualitative} for a discussion.}
%\label{fig:qualitative_CoHRE}
%\vspace{-0.5cm}
%\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{fig/teaser.png}
    \caption{A glimpse on the \dataname{} dataset and a collision example. On the first row some frames of the \emph{Lightweight pick and place} action captured by one of the three cameras. On the second row, operator + robot skeletons. The forecasting takes an observation sequence (in yellow, here portrayed for the right wrist only), and perform a prediction (cyan) which is compared with the ground truth (green). On frame 395 is it easy to see the robot hitting the operator, which is retracting as evident in frame 421.}\MC{Forse meglio mostrare il nostro forecasting... mostrare marker di tipo diversi e citare SES-GCN}
    \label{fig:teaser}
\end{figure}

Collaborative robots (cobots) and modern Human Robot Collaboration (HRC) depart from the traditional separation of functions of industrial robots~\cite{Stein2020}, since cobots share the same workspace as the human workers~\cite{iso15066}. Additionally cobots and humans perform actions concurrently and they will therefore physically engage in contact. While there is a clear advantage in increased productivity~\cite{Rodriguez-Guerra2021} (improved by as much as 85\%~\cite{Shah2011}) due to the minimization of idle times, there are challenges in the workplace safety~\cite{Gualtieri2020}: it is not about whether there will be contact, but rather about understanding its consequences~\cite{Matthias2016}.



The pioneering work of Shah et al.~\cite{Shah2011} has already shown that, in order to seamlessly and efficiently interact with human co-workers, cobots need to abide by two collaborative principles: \textbf{i.}\ Making decisions on-the-fly, and \textbf{ii.}\ Considering the consequences of their decision on their teammates. The first calls for promptly and accurately detecting the human motion in the workspace. The second principle implies that cobots need to anticipate pose trajectories of their human co-workers and predict future collisions. \MC{maybe 1 and 2 instead of i and ii?}



Motivated by these problems, the first contribution of our work is a novel Separable-Sparse Graph Convolutional Neural Network (\gcnname{}) for human pose forecasting. Pose forecasting requires understanding of the complex spatio-temporal joint dynamics of the human body and recent trends have highlighted the promises of modelling body kinematics within a single GCN framework \cite{Dang21,li21,Wang_21,Zhao20,cui20,li20,Mao19LTD}.
We have designed \gcnname{} with performance and efficiency in mind, by bringing together, for the first time, three main modelling principles: depthwise-separable graph convolutions~\cite{lai18}, space-time separable graph adjacency matrices ~\cite{stsgcn}, and sparse graph adjacency matrices~\cite{shi21}.
In \gcnname{}, \emph{separable} stands for limiting the interplay of joints with others (space), at different frames (time) and per channel (depth-wise). Within the GCN, different channels, frames and joints still interact by means of multi-hop messages, i.e.\ messages take 2 layers to be delivered.
For the first time, sparsity is achieved by a teacher-student framework.
The reduced interaction and sparsity results in considerably fewer parameters (4x less), so \gcnname{} is lightweight, fast ($\sim$5 msec runtime) \AS{cambiare posizione FABIO, dire solamente che siamo molto veloci, negligible rispoetto a...}, and ultimately accurate, i.e.\ it outperforms the state-of-the-art (SoA)~\cite{stsgcn} by 3.6\% on Human 3.6M~\cite{h36m_pami} when predicting at 1 sec in the future. The model is described in detail in Sec.~\ref{sec:methodology}, experiments and ablation studies are illustrated in  Sec.~\ref{sec:experimental_results_h36m}.
%Our model is the first GCN to use a teacher-student sparsification framework and the first fully separable GCN in space, time and channels. \gcnname{} results in a lightweight and deep model, mindful of the over-smoothing~\cite{Oono20} problem, and is described in detail in Sec.~\ref{sec:methodology}.



%%MARCO:https://journals.sagepub.com/doi/abs/10.1177/02783649211050677?journalCode=ijra  dataset HR
We also introduce the very first benchmark of Cobots and Humans in Industrial COllaboration (\dataname{}).
%where safety plays a crucial role.
\dataname{} includes multi-view videos, 3D poses and trajectories of the joints of 20 human operators, in close collaboration with a robotic arm \emph{KUKA LBR iiwa} within a shared workspace. The dataset features 8 realistic industrial actions, taken at a real industrial assembly line with a marker-less setup.
%The recorded human actions are fine-grained (e.g.\ lifting objects from the ground and placing them on a table close to the cobot \FG{report a better example of fine grained, eg small-large range, clock-wise-anti-clockwise, or mention the reduced workspace?}) and therefore demand minimal trajectory forecasting error to be discerned \FG{but no activity recognition is pursued}.
The goal of \dataname{} is to endow cobots with perceptive awareness to enable human-cobot collaboration with contact. Towards this frontier, \dataname{} proposes to benchmark two key tasks: human pose forecasting and collision detection.
Cobots currently detect collisions by mechanical-only events (transmission of contact wrenches, control torques, sensitive skins). This ensures safety but it harms the human-cobot interaction, because collisions break the motion of both, which reduces productivity, and may be annoying to the human operator.
%The additional aim of \dataname{} is to bring safety in HRC at another level, in which collisions are not detected by mechanical events (transmission of contact wrenches, control torques, sensitive skins), but foreseen by visual forecasting. In fact, mechanical events imply that the collision does happen; on the contrary, we want to predict it \emph{before} it happens. \FG{I can't be convinced on the argument on safety. These robots ARE safe, else we could not test them/ask anyone to record these experiments. However collisions are time-consuming, break concentration, and are anti-social (anti-colab), not sustainable in industry in the long term.}
%%MARCO https://d-nb.info/1211397823/34
%To this sake, \dataname{} contains ZZ genuine collisions generated by  consensual human operators collaborating on quick activities with the cobot choosing randomly its routines from one point to another \FG{randomly? maybe mention arbitrary decisions and multi-modality, eg humans have multiple pathways and start/stop moments to move things from A to B, even if the action is carefully scripted. In a h-cobot scenario the collision will occur, unless both parties watch out for the "intention" of the other}. Despite collisions are real, it is worth noting that they were harmless, since the cobot was setup to have maximum sensibility, and the actions were designed to have the right arm of the human operator potentially colliding with the robot. 
%The data acquisition process, as well as ethical issues and limitations of \dataname{} are discussed in Sec.~\ref{sec:cohre_dataset}.
\dataname{} features 160 3-minute video recordings, from which two separate sets of test sequences are selected: one for estimating the accuracy in pose forecasting, so cobots may be aware of the next future (1.2 sec); and one with 158 genuine collisions, so cobots may foresee them and possibly re-plan.
The dataset is detailed in Sec.~\ref{sec:cohre_dataset}, experiments are illustrated in  Sec.~\ref{sec:experimental_results_sd}.

When tested on \dataname{}, the proposed \gcnname{} outperforms all baselines and reaches an error of \FG{57.3}$mm$ (MPJPE) at \FG{1.2} sec, with negligible runtime. 
Additionally, the forecast human motion is used to detect human-cobot collision, by checking whether the predicted trajectory of the human body intersects that of the cobot. This is also encouraging, as \gcnname{} allows to reach an F1-score of \MC{X}.
Both aspects contribute to a cobot awareness of the future, which is instrumental for HRC in industrial applications.



==> src/Backup/method_bk_2022-03-04.tex <==
We build a ``fully-separable'' Graph Convolutional Network by considering three ideas on how a GCN may be improved in terms efficiency and, as we show, in accuracy: \textbf{i.}\ Depth-wise separable convolutions; \textbf{ii.}\ Space-time separable adjacency matrices; \textbf{iii.}\ Sparse adjacency matrices.
In all cases body kinematics are encoded by a GCN and then the future is forecast using a Temporal Convolutional Network (TCN).
\FG{Novelty? Say that (i) is novel for GCN, and that (ii) and (iii) have not been adopted within the same model/these are orthogonal model compression ideas, which we analyze. Add that we target a fast and memory-efficient model, we take the fastest and most-memory efficient model available (sts-gcn), and we target its improvement, by 2 principles for accuracy: more depth, more separability; and by 1 principle for memory-efficiency: sparsity}


\subsection{Background}
Pose forecasting is formulated as observing the 3D coordinates $\boldsymbol{x}_{v,t}$ of $V$ joints across $T$ frames and predicting the location of said joints in the $K$ future frames. For convenience of notation, we gather the coordinates from all joints at frame $t$ into the matrix $X_t=\left[ \boldsymbol{x}_{v,t} \right]_{v=1}^{V} \in \mathbb{R}^{3 \times V}$. Then we define the tensors $\mathcal{X}_{in}=[X_1,X_2...,X_T]$ and $\mathcal{X}_{out}=[X_{T+1},X_{T+2}...,X_{T+K}]$ that contain all observed input and target frames, respectively.



The relation of body joints across time can be encoded as a graph  $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where the node set is given by all joints across all observed frames $\mathcal{V}=\left\{ \boldsymbol{v}_{i,t} \right\}_{i=1,t=1}^{V,T}$, and edges $(\boldsymbol{v}_{i,t},\boldsymbol{v}_{j,s})\in \mathcal{E}$ that connect nodes $i, j$ on frames $t, s$. This allows the use of GCNs to encode the information of body joints across time. The base GCN is a layered architecture, repeating the basic operation:
\begin{equation}
\mathcal{X}^{(l+1)} = \sigma\left(A^{(l)} \mathcal{X}^{(l)} W^{(l)}\right)
\label{eq:gcn}
\end{equation}

The input to a Graph Convolutional Layer $l$ is the tensor $\mathcal{X}^{(l)} \in \mathbb{R}^{C^{(l)} \times V \times T}$ which maintains the correspondence to the $V$  body joints and the $T$ observed frames, but increases the depth of features to $C^{(l)}$ channels, varying for each layer $l$. $\mathcal{X}^{(1)}=\mathcal{X}_{in}$ is the input tensor at the first layer, with $C^{(1)}=3$ channels given by the 3D coordinates. $A \in \mathbb{R}^{VT\times VT}$ is the adjacency matrix relating pairs of $VT$ joints from all frames. Former literature \cite{Yan18stgcn} has adopted block diagonal $A$ matrices, set to 1 for neighbor joints along the kinematic tree and on adjacent frames, and 0 otherwise. More recent literature \cite{Mao20DCT} has regarded $A$ as a learnable parameter. When $A$ is an unconstrained learnable parameter, the resulting graph is generally signed  and directed (due to an asymmetric $A$)\cite{stsgcn,shi21}. $W^{(l)}$ are the weights of the graph convolutional layer $l$ that maps the channels of each node from $C^{(l)}$ to $C^{(l+1)}$. Finally, $\sigma$ is an (typically non-linear) activation function.

\subsection{Separable Sparse Graph Convolutional Networks}

We propose the adoption of a novel ``fully-Separable'' GCN that segregates the interplay of different body joints from different frames and different channels. The novel graph convolutional layer is formulated as follows:
\begin{subequations}
\begin{align}
\mathcal{H}^{(l)} =&  \sigma\left(A^{s-(l)} A^{t-(l)} \mathcal{X}^{(l)} W_{DW}^{(C-l)}\right) \label{eq:sepgcn}\\
\mathcal{X}^{(l+1)} &= \gamma\left(\mathcal{H}^{(l)} W^{(l)}\right) \label{eq:mlp}
\end{align}
\end{subequations}



Where the spatial adjacency matrix $A^{s}\in\mathbb{R}^{V\times V\times T}$ represents the relationships among joints for each temporal step and the temporal adjacency matrix $A^{t}\in\mathbb{R}^{T\times T\times V}$ is responsible for the temporal relationships between a joint with itself. $W_{DW}^{(C-l)}$  is a further separation at the channel level and represents a depthwise convolution. This operation allows minimal memory usage and efficiency by using the same filter for each node feature. %Thus, in equation \ref{eq:sepgcn} a non-linearity is adopted. 
The encoded data tensor $\mathcal{X}^{(l+1)}$ for layer $l+1$ is then derived as in equation \ref{eq:mlp}, with $\gamma$ identifying a non-linear activation function and $ W^{(l)}$ denoting an MLP applied to each graph node, mapping features from $C^{(l)}$ to $C^{(l+1)}$. 




Finally the proposed Separable-Sparse GCN (SeS-GCN) is obtained by applying sparsity to the graph adjacency matrices $A^{s}$ and $A^{t}$, to further reduce the number of parameters. This is motivated by SGCN \cite{shi21}, that sparsifies adjacency matrices, but it is here applied to a factored graph adjacency matrix for the first time.
We formulate the separable sparsification by replacing Eq.\ref{eq:sepgcn} with the novel term:% \ref{eq:SeSlayer}.

\begin{equation}
\mathcal{H} = \sigma\left( (\mathcal{M}^{s} \odot A^{s})( \mathcal{M}^{t}\odot A^{t}) \mathcal{X} W_{DW}^{(C)}\right) \label{eq:SeSlayer}
\end{equation}
\noindent
with $\odot$ being the element-wise product and $\mathcal{M}^{\{s,t\}}$ a binary mask. Eq.\ref{eq:SeSlayer} represents a single SeS-GCN layer in which a factorization of the adjacency matrix takes place, whereby the intra-time and intra-joints connections are further reduced. 




The procedure to obtain these masks involves two steps: initially, a first generation of the model is trained from scratch, leaving it free to learn the adjacency relationships between nodes. Then a mask is derived by applying to each learned matrix $A^{\{s,t\}-(l)}$ a hyperbolic tangent and cutting-off connections below a threshold $\varepsilon$:
\begin{equation}
\mathcal{M}^{\{s,t\}-(l)} = \mathbb{I}\{ |\tanh(A^{\{s,t\}-(l)})| \ge \varepsilon\}
\label{eq:mask}
\end{equation}
where $\mathbb{I}$ is the characteristic function. \\

Thus formulated, SeS-GCN bottlenecks its adjacency connections, which forces the network to rely only on few-but-robust affinities. Moreover, this design allows us to build a deeper network while maintaining a lightweight parametrization, removing up to 25\% of $A^{s-(l)}$ and $A^{t-(l)}$ connections.
\subsection{Decoder Forecasting}
Given the encoded space-time representation, SeS-GCN decodes future frames using a temporal convolutional network (TCN) \cite{Bai18TCN,Gehring17,Li18}, which expands the temporal dimension through its architecture. The use of a convolutional structure contributes to parameter containment when compared to recurrent models such as RNNs \cite{gru14,lstm97} or Transformers \cite{VaswaniAttention,giuliari20}.



\subsection{Collision forecasting}

To predict whether there will be a collision between human and robot in the forecasting horizon we adapted an approach proposed in~\cite{minelli2020iros}. We model both the agents as a composition of capsules, that enclose each limb into the fittest and simplest shape. 
Given  a  pair  of  Cartesian  points,  a  capsule  is  an object composed by two hemispheres, centered in that points, and a cylinder, with longitudinal axis linking the two points.
\MC{Francesco, spostare a 6.2}

==> src/Backup/method_bk_2022-03-06.tex <==
We build a ``fully-separable'' Graph Convolutional Network by considering three ideas on how a GCN may be improved in terms efficiency and, as we show, in accuracy: \textbf{i.}\ Depth-wise separable convolutions; \textbf{ii.}\ Space-time separable adjacency matrices; \textbf{iii.}\ Sparse adjacency matrices.
In all cases body kinematics are encoded by a GCN and then the future is forecast using a Temporal Convolutional Network (TCN).
\FG{Novelty? Say that (i) is novel for GCN, and that (ii) and (iii) have not been adopted within the same model/these are orthogonal model compression ideas, which we analyze. Add that we target a fast and memory-efficient model, we take the fastest and most-memory efficient model available (sts-gcn), and we target its improvement, by 2 principles for accuracy: more depth, more separability; and by 1 principle for memory-efficiency: sparsity}

% space-time-depthwise-separable and sparse GCN

\subsection{Background}

%Potremmo spezzare il background in due sotto paragrafi: 
% 1. Problem Formalization
\myparagraph{Problem Formalization.} Pose forecasting is formulated as observing the 3D coordinates $\boldsymbol{x}_{v,t}$ of $V$ joints across $T$ frames and predicting the location of said joints in the $K$ future frames. For convenience of notation, we gather the coordinates from all joints at frame $t$ into the matrix $X_t=\left[ \boldsymbol{x}_{v,t} \right]_{v=1}^{V} \in \mathbb{R}^{3 \times V}$. Then we define the tensors $\mathcal{X}_{in}=[X_1,X_2...,X_T]$ and $\mathcal{X}_{out}=[X_{T+1},X_{T+2}...,X_{T+K}]$ that contain all observed input and target frames, respectively.

The relation of body joints across time can be encoded as a graph  $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where the node set is given by all joints across all observed frames $\mathcal{V}=\left\{ \boldsymbol{v}_{i,t} \right\}_{i=1,t=1}^{V,T}$, and edges $(\boldsymbol{v}_{i,t},\boldsymbol{v}_{j,s})\in \mathcal{E}$ that connect nodes $i, j$ on frames $t, s$. This allows the use of GCNs to encode the information of body joints across time. 
% 2. GCN
\smallskip
\myparagraph{Graph Convolutional Networks.}
The base GCN is a layered architecture, repeating the basic operation:
\begin{equation}
\mathcal{X}^{(l+1)} = \sigma\left(A^{(l)} \mathcal{X}^{(l)} W^{(l)}\right)
\label{eq:gcn}
\end{equation}

The input to a Graph Convolutional Layer $l$ is the tensor $\mathcal{X}^{(l)} \in \mathbb{R}^{C^{(l)} \times V \times T}$ which maintains the correspondence to the $V$  body joints and the $T$ observed frames, but increases the depth of features to $C^{(l)}$ channels. $\mathcal{X}^{(1)}=\mathcal{X}_{in}$ is the input tensor at the first layer, with $C^{(1)}=3$ channels given by the 3D coordinates. $A \in \mathbb{R}^{VT\times VT}$ is the adjacency matrix relating pairs of $VT$ joints from all frames. Former literature \cite{Yan18stgcn} has adopted block diagonal $A$ matrices, set to 1 for neighbor joints along the kinematic tree and on adjacent frames, and 0 otherwise. More recent literature \cite{Mao20DCT,stsgcn,shi21} has regarded $A$ as a learnable parameter.
%When $A$ is an unconstrained learnable parameter, the resulting graph is generally signed  and directed (due to an asymmetric $A$)\cite{stsgcn,shi21}.
$W^{(l)}$ are the weights of the graph convolutional layer $l$ that maps the channels of each node from $C^{(l)}$ to $C^{(l+1)}$. Finally, $\sigma$ is an (typically non-linear) activation function.


\subsection{Separable Sparse Graph Convolutional Networks}

\FG{too much background above, too little and intertwined contribution from us here. Need to to explode this section more, at least adding two paragraphs to separate the separable and the sparse extension. It'd be ideal to have 3 paragraphs here, corresponding to the 3 ideas metioned in input (i, ii, iii). Need to keep in mind that we need to better separate our work from sts-gcn and from sgcn. Having everything mixed is not helping.}
%We propose the adoption of a novel ``fully-Separable'' GCN that segregates the interplay of different body joints from different frames and different channels. 
%
Recent literature has demonstrated the benefit of adopting separability between the spatial and temporal dimensions both in human pose  related tasks~\cite{Yan18stgcn,stsgcn}, and in the similar domain of social trajectory forecasting~\cite{shi21,mohamed2020social}. Our work fits into this framework by proposing the first "fully-Separable" GCN that extends separation over the channel dimension, thanks to lightweight depth-wise convolutions. Moreover, we reinforced the learning process by exploiting a teacher-student procedure to introduce targeted sparsity into the model, selecting only the most robust spatio-temporal connections. We will describe in detail the different modules of the proposed Separable-Sparse GCN (SeS-GCN) in the following paragraphs.
%

\smallskip
\myparagraph{DW Separable GCN.} Aiming to reduce the model complexity while keeping good performances, we leveraged Graph DepthWise Convolutions which applies a separation at the channels level. This operation allows minimal memory usage and efficiency by using the same filter for each node feature, and has been shown to be effective in~\cite{lai18} for image classification and time series forecasting. With similar notation to Eq.\ref{eq:gcn}, the graph DW-convolutional layer can be formulated as follows:

\begin{equation}
\mathcal{H}^{(l)} =  \sigma\left(A \mathcal{X}^{(l)} W_{DW}^{C,(l)}\right) \label{eq:sepgcn}
\end{equation}
%
\smallskip
\myparagraph{Separable GCN.} Separability has shown to be effective in training GCN on space-time dependent data [X,Y,Z]. Separate the spatial adjacency matrix from the temporal one avoids the cross-talk and improves the stability of predictions. It causes a reduction in the model parameters wrt a vanilla GCN by the use of two dedicated matrices $A_s\in\mathbb{R}^{V\times V\times T}$ and $A_t\in\mathbb{R}^{T\times T\times V}$, which are responsible for the spatial intra-frame connections and the temporal per joint relationship, respectively. Our proposed model separates over all the input dimensions, being to the best of our knowledge the first fully-Separable GCN. We can formalize a single fully-separable GCN layer (indexed with $l$) as follows:

% The novel graph convolutional layer is formulated as follows:

%secondo me senza le l nelle formule sono più leggibili

\begin{equation}
\mathcal{H}^{(l)} =  \sigma\left(A^{(l)}_s A^{(l)}_t \mathcal{X}^{(l)} W_{DW}^{C,(l)}\right) \label{eq:sepgcn}%\\
%\mathcal{X}^{(l+1)} &= \gamma\left(\mathcal{H}^{(l)} W^{(l)}\right) \label{eq:mlp}
\end{equation}
The encoded data tensor $\mathcal{X}^{(l+1)}$ for layer $l+1$ is then derived as in equation \ref{eq:mlp}, with $\gamma$ identifying a non-linear activation function and $ W^{(l)}$ denoting an MLP applied to each graph node, mapping features from $C^{(l)}$ to $C^{(l+1)}$.
\begin{equation}
\mathcal{X}^{(l+1)} = \gamma\left(\mathcal{H}^{(l)} W^{(l)}\right) \label{eq:mlp}
\end{equation}

% \begin{subequations}
% \begin{align}
% \mathcal{H}^{(l)} =&  \sigma\left(A^{s,(l)} A^{t, (l)} \mathcal{X}^{(l)} W_{DW}^{(C-l)}\right) \label{eq:sepgcn}\\
% \mathcal{X}^{(l+1)} &= \gamma\left(\mathcal{H}^{(l)} W^{(l)}\right) \label{eq:mlp}
% \end{align}
% \end{subequations}

% Where the spatial adjacency matrix $A^{s}\in\mathbb{R}^{V\times V\times T}$ represents the relationships among joints for each temporal step and the temporal adjacency matrix $A^{t}\in\mathbb{R}^{T\times T\times V}$ is responsible for the temporal relationships between a joint with itself. $W_{DW}^{(C-l)}$  is a further separation at the channel level and represents a depthwise convolution. This operation allows minimal memory usage and efficiency by using the same filter for each node feature. %Thus, in equation \ref{eq:sepgcn} a non-linearity is adopted. 
% The encoded data tensor $\mathcal{X}^{(l+1)}$ for layer $l+1$ is then derived as in equation \ref{eq:mlp}, with $\gamma$ identifying a non-linear activation function and $ W^{(l)}$ denoting an MLP applied to each graph node, mapping features from $C^{(l)}$ to $C^{(l+1)}$. 
\smallskip
\myparagraph{Sparse GCN.}
Finally the proposed Separable-Sparse GCN (SeS-GCN) is obtained by applying sparsity to the graph adjacency matrices $A_{s}$ and $A_{t}$, to further reduce the number of parameters. This is motivated by SGCN~\cite{shi21}, that sparsifies adjacency matrices, but it is here applied to a factored graph adjacency matrix for the first time \AS{anche SGCN ha una matrice As e una At.. siamo i primi a farlo in pose forecasting e i primi a fine train}.
We formulate the separable sparsification by replacing Eq.~\ref{eq:sepgcn} with the novel term:% \ref{eq:SeSlayer}.
\begin{equation}
\mathcal{H} = \sigma\left( (\mathcal{M}_{s} \odot A_{s})( \mathcal{M}_{t}\odot A_{t}) \mathcal{X} W_{DW}^{(C)}\right) \label{eq:SeSlayer}
\end{equation}
\noindent
with $\odot$ being the element-wise product and $\mathcal{M}_{\{s,t\}}$ a binary mask. Eq.~\ref{eq:SeSlayer} represents a single SeS-GCN layer in which a factorization of the adjacency matrix takes place, whereby the intra-time and intra-joints connections are further reduced. 




The procedure to obtain these masks involves two steps: initially, a first generation of the model is trained from scratch, leaving it free to learn the adjacency relationships between nodes. Then a mask is derived by applying to each learned matrix $A_{\{s,t\}}{(l)}$ a hyperbolic tangent and cutting-off connections below a threshold $\varepsilon$:
\begin{equation}
\mathcal{M}_{\{s,t\}}^{(l)} = \mathbb{I}\{ |\tanh(A_{\{s,t\}}^{(l)})| \ge \varepsilon\}
\label{eq:mask}
\end{equation}
where $\mathbb{I}$ is the characteristic function. \\

Thus formulated, SeS-GCN bottlenecks its adjacency connections, which forces the network to rely only on few-but-robust affinities. Moreover, this design allows us to build a deeper network while maintaining a lightweight parametrization, removing up to 34.4\% and 28.4\% of $A_s$ and $A_t$ original connections, respectively.


\subsection{Decoder Forecasting}

Given the space-time representation, as encoded by the SeS-GCN, the future frames are then decoded by using a temporal convolutional network (TCN)~\cite{Bai18TCN,Gehring17,Li18}. The TCN remaps the temporal dimension to match the sought output number of predicted frames.
The use of a convolutional structure contributes to parameter containment when compared to recurrent models such as RNNs \cite{gru14,lstm97} or Transformers \cite{VaswaniAttention,giuliari20}. \FG{Comment on why we don't consider this for model compression, cf rebuttal.}





==> src/discussion.tex <==

\begin{minipage}{.6\textwidth}
    
      \centering
      \resizebox{\linewidth}{!}{
        \begin{tabular}{|l|c|c|c|c|c|c|}
          \hline
          \textit{Time Horizon (msec)} & \multicolumn{3}{c|}{500} & \multicolumn{3}{c|}{1250} \\ \hline
          Metrics & prec & recall & F$_1$ & prec & recall & F$_1$ \\ \hline
          DCT-RNN-GCN~\cite{Mao20DCT} &  &  &  &  &  &  \\
          MSRGCN~\cite{Dang21} &  &  &  &  &  &  \\
          STS-GCN~\cite{stsgcn} &  &  &  &  &  &  \\ \hline
          \gcnname &  &  &  &  &  &  \\ \hline
        \end{tabular}
      }
      \captionof{table}{Collision detection performances }
      \label{tab:collisions}
\end{minipage}%
\begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{fig/roc_collisions.png}
    \captionof{figure}{ToDO}
    \label{fig:roc_collision}
\end{minipage}

==> tab/amass_quantitative.tex <==
\begin{table}[!htb]
\centering
\begin{tabular}{c|cc|}
\cline{2-3}
                                          & \multicolumn{2}{c|}{AMASS-BMLrub}     \\ \hline
\multicolumn{1}{|c|}{Time Horizon (msec)} & {\ul \textit{400}} & {\ul \textit{1000}}              \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT} }       & 42.0              & 67.2              \\
\multicolumn{1}{|c|}{MSRGCN \cite{Dang21}   }     & ---               & ---               \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}         & \textbf{24.3}           & \textbf{44.7}              \\ \hline
\multicolumn{1}{|c|}{Ours}                & 25.5 & 46.7 \\ \hline
\end{tabular}
\caption{Caption}
\label{tab:amass_quantitative}
\end{table}

==> tab/h36m_quantitative.tex <==
\begin{table}[]
\centering

\begin{tabular}{|c|cc|}
\cline{2-3}
\multicolumn{1}{c|}{}     & \multicolumn{2}{c|}{Average}     \\                             
\hline
\textit{msec} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
DCT-RNN-GCN \cite{Mao20DCT}   & 58.3               & 112.1               \\
MSRGCN \cite{Dang21}       & 62.9               & 114.1*               \\
STS-GCN \cite{stsgcn}     & 38.3               & 75.6                \\ \hline
Ours          & \textbf{37.6}               & \textbf{73.8}                \\ \hline
\end{tabular}
\caption{}
\label{tab:h36m_quantitative}
\end{table}

==> tab/tab_vecchie/3dpw_quantitative.tex <==
\begin{table}[!htb]
\centering
\begin{tabular}{c|cc|}
\cline{2-3}
                                          & \multicolumn{2}{c|}{3DPW}             \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}}              \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}  }       & 45.4              & 73.7              \\
\multicolumn{1}{|c|}{MSRGCN \cite{Dang21}  }            & ---               & ---               \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn} }           & \textbf{24.5}              & \textbf{42.3}              \\ \hline
\multicolumn{1}{|c|}{Ours}                & 24.9 & 43.0 \\ \hline
\end{tabular}
\caption{Caption}
\label{tab:3dpw_quantitative}
\end{table}

==> tab/tab_vecchie/CHICO_comparative_BAK.tex <==

\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
%\begin{tabular}{l|ccccccc|c|ccc|c|}
%\cline{2-13}
\begin{tabular}{l|ccccccc|c|cc|ccc|c|}
\cline{2-15}
\multirow{2}{*}{} &
  \multicolumn{7}{c|}{\textbf{Quantitative Details}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Rec.\\ Scene\end{tabular}}} &
  \multicolumn{2}{c|}{\textbf{Actions Type}} &
  \multicolumn{3}{c|}{\textbf{Tasks}} &
  \multirow{2}{*}{\textbf{Markerless}}  \\ \cline{2-8} \cline{10-11} \cline{12-14} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\#\\ Classes\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\#\\ Subj.\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg Rec.\\  Time\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\#\\ Joints\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{FPS}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Aspect\\ Ratio\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\# \\  Sensors\end{tabular}} &
   &
\multicolumn{1}{c|}{\textbf{Industr.}} &
\multicolumn{1}{c|}{\textbf{HRC}} &
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Action\\ Recog.\end{tabular}}} &
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Pose\\ Forec.\end{tabular}}} &
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Coll.\\ Det.\end{tabular}}} &
   \\ \hline

\multicolumn{1}{|l|}{Human3.6M ~\cite{h36m_pami}} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{100.49 s} &
  \multicolumn{1}{c|}{32} &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{normalized} &
  15 &
  \begin{tabular}[c]{@{}c@{}}mo-cap\\ studio\end{tabular} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark}
   & &\\ \hline
 %  
   
  \multicolumn{1}{|l|}{AMASS~\cite{AMASS:ICCV:2019}} &
  \multicolumn{1}{c|}{11265} &
  \multicolumn{1}{c|}{344} &
  \multicolumn{1}{c|}{12.89 s} &
  \multicolumn{1}{c|}{variable} &
  \multicolumn{1}{c|}{variable} &
  \multicolumn{1}{c|}{original} &
  variable &
  \begin{tabular}[c]{@{}c@{}}mo-cap\\ studio\end{tabular} &
 \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark}
   & &\\ \hline
   %
   
\multicolumn{1}{|l|}{3DPW~\cite{vonMarcard2018}} &
  \multicolumn{1}{c|}{47} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{28.33 s} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{original} &
  18 &
  \begin{tabular}[c]{@{}c@{}}outdoor\\ locations\end{tabular} &
 \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark}
   & &\\ \hline
   %
    
\multicolumn{1}{|l|}{ExPI~\cite{guo2021multi}} &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{\emph{unk}} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{original} &
  88 &
  \begin{tabular}[c]{@{}c@{}}mo-cap\\ studio\end{tabular} &
 \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark}
   & &\\ \hline

 %  
\multicolumn{1}{|l|}{CHI3D~\cite{fieraru2020three}} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{\emph{unk}} &
  \multicolumn{1}{c|}{\emph{unk}} &
  \multicolumn{1}{c|}{\emph{unk}} &
  \multicolumn{1}{c|}{original} &
  14 &
  \begin{tabular}[c]{@{}c@{}}mo-cap \\ studio\end{tabular} &
 \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark}
   & &\\ \hline
   %
  
\multicolumn{1}{|l|}{InHARD~\cite{Dallel2020}} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{$<$ 8 s} &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{120} &
  \multicolumn{1}{c|}{original} &
  20 &
  \begin{tabular}[c]{@{}c@{}}assembly \\ line\end{tabular} &
%  \multicolumn{1}{c|}{\checkmark} &
   \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{}
   & &\\ \hline    \hline
   %
     %   \iffalse
 \multicolumn{1}{|l|}{\dataname (ours)} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{180.24 s} &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{original} &
  3 &
  \begin{tabular}[c]{@{}c@{}}assembly \\ line\end{tabular} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{\checkmark} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\checkmark}
   &\checkmark &\checkmark\\ \hline    %\hline
%\fi
 % \hline
\end{tabular}%
}

\caption{Comparison between the state-of-the-art datasets and the proposed \dataname; \emph{unk} stands for ``unknown''. %\MC{non sono convinto delle colonne Industrial e HRC... ci devo pensare}
%\FG{Remove daily actions. Leave only Industrial and HRC. Add a super column "Tasks", with two sub-columns "Action Recog." and "Pose Forecasting" and "collision detection"}
}
\label{tab:symbiotic_h36_comparative}
\vspace{-0.9cm}
\end{table*}


==> tab/tab_vecchie/CHICO_quantitative_full.tex <==
\begin{table}[]
\centering
\resizebox{1.\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-19}
                                          & \multicolumn{2}{c|}{Low Lift} & \multicolumn{2}{c|}{Hammer}   & \multicolumn{2}{c|}{High Lift} & \multicolumn{2}{c|}{Prec. P\emph{\&}P} & \multicolumn{2}{c|}{Rnd. P\emph{\&}P} & \multicolumn{2}{c|}{Polishing} & \multicolumn{2}{c|}{Heavy P\emph{\&}P} & \multicolumn{2}{c|}{Light P\emph{\&}P} & \multicolumn{2}{c|}{Average}  \\ \hline
\multicolumn{1}{|l|}{\textit{Time Horizon (msec)}} & {\ul \textit{500}  }         & {\ul \textit{1250} }          & {\ul \textit{500}}           & {\ul \textit{1250} }      & {\ul \textit{500}}           & {\ul \textit{1250}   }      &{\ul \textit{500}     }      & {\ul \textit{1250}   }      & {\ul \textit{500}  }         & {\ul \textit{1250}   }   & {\ul \textit{500}  }         & {\ul \textit{1250} }        & {\ul \textit{500}  }         & {\ul \textit{1250}}    & {\ul \textit{500}}           & {\ul \textit{1250}}       & {\ul \textit{500} }          & {\ul \textit{1250} }       \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}         & 85.2          & 143.5         & \textbf{41.7} & \textbf{37.9} & 34.2           & 64.8          & 36.8           & 70.7           & 26.4           & 47.6          & 36.6           & 81.2          & 52.5           & 94.5           & 39.6           & 71.2           & 44.1          & 76.4          \\
\multicolumn{1}{|c|}{MSR-GCN \cite{Dang21}}              & 297.2         & 302.1         & 182.3         & 202.3         & 49.5           & 60.4          & 76.6           & 102.7          & 50.4           & 60.8          & 124.5          & 147.8         & 115.6          & 130.3          & 57.4           & 85.7           & 119.1         & 136.5         \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}             & 61.7          & 110.5         & 79.1          & 101.0         & 28.5           & 48.3          & 29.0           & \textbf{42.6}  & 23.4           & 33.9          & 35.1           & 58.2          & 37.7           & 63.3           & 28.3           & 47.8           & 36.7          & 59.0          \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}                & \textbf{52.3} & \textbf{97.5} & 58.9          & 85.7          & \textbf{22.3}  & \textbf{41.5} & \textbf{22.0}  & 44.1           & \textbf{17.5}  & \textbf{33.2} & \textbf{25.1}  & \textbf{48.9} & \textbf{30.0}  & \textbf{55.9}  & \textbf{23.2}  & \textbf{44.3}  & \textbf{28.7} & \textbf{53.0} \\ \hline
\end{tabular}
}
\caption{ MPJPE error in mm for short-term (500 msec, 10 frames) and long-term (1250 msec, 25 frames) prediction of 3D joint positions on \dataname dataset. Our SeS-GCN outperforms particularly better for complex actions such as Heavy P\emph{\&}P and High Lift for which two hands are required. The average error is 21.8\% lower than the other models in the short-term and 10.1\% lower in the long-term prediction. See Sec.\ref{subsec:quantitative_symb} for a discussion.}
\label{tab:CHICOresults}
\vspace{-.3cm}
\end{table}

==> tab/tab_vecchie/Symbiotic_quantitative.tex <==
\begin{table*}[!ht]
\centering
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-15}
                                 & \multicolumn{2}{c|}{Crash heavy} & \multicolumn{2}{c|}{Crash light} & \multicolumn{2}{c|}{Crash polish} & \multicolumn{2}{c|}{Ground} & \multicolumn{2}{c|}{Hammer} & \multicolumn{2}{c|}{Lift} & \multicolumn{2}{c|}{Place high p.} \\ \hline
\multicolumn{1}{|c|}{{\ul msec}} & {\ul 660}      & {\ul 1660}      & {\ul 660}      & {\ul 1660}      & {\ul 660}       & {\ul 1660}      & {\ul 660}    & {\ul 1660}   & {\ul 660}    & {\ul 1660}   & {\ul 660}   & {\ul 1660}  & {\ul 660}       & {\ul 1660}       \\ \hline
\multicolumn{1}{|c|}{STS-GCN}    & 19.3           & 35.9            & 19.9           & 37.0            & 15.0            & 26.1            & 20.2         & 39.4         & 20.4         & 30.9         & 20.0        & 40.7        & 15.9            & 29.2             \\
\multicolumn{1}{|c|}{SeS-GCN}    & 16.4           & 33.7            & 16.8           & 35.2            & 12.3            & 22.5            & 17.5         & 36.9         & 18.5         & 28.9         & 16.7        & 33.3        & 14.2            & 27.4             \\ \hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|}
\cline{2-13}
                                 & \multicolumn{2}{c|}{Place low p.} & \multicolumn{2}{c|}{Polish} & \multicolumn{2}{c|}{Span heavy} & \multicolumn{2}{c|}{Span Light} & \multicolumn{2}{c|}{Table} & \multicolumn{2}{c|}{Average} \\ \hline
\multicolumn{1}{|c|}{{\ul msec}} & {\ul 660}       & {\ul 1660}      & {\ul 660}    & {\ul 1660}   & {\ul 660}      & {\ul 1660}     & {\ul 660}      & {\ul 1660}     & {\ul 660}   & {\ul 1660}   & {\ul 660}    & {\ul 1660}    \\ \hline
\multicolumn{1}{|c|}{STS-GCN}    & 14.2            & 28.8            & 14.8         & 25.8         & 16.1           & 31.5           & 8.6            & 17.1           & 21.6        & 41.1         & 17.3         & 32.2          \\
\multicolumn{1}{|c|}{SeS-GCN}    & 12.8            & 27.1            & 12.7         & 23.3         & 13.6           & 29.4           & 7.8            & 15.5           & 18.5        & 36.9         & 14.9         & 29.4          \\ \hline
\end{tabular}
\end{table*}



==> tab/tab_vecchie/Symbiotic_quantitative_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-27}
                                    & \multicolumn{2}{c|}{Crash heavy}         & \multicolumn{2}{c|}{Crash light}         & \multicolumn{2}{c|}{Crash polish}        & \multicolumn{2}{c|}{Ground}              & \multicolumn{2}{c|}{Hammer}              & \multicolumn{2}{c|}{Lift}                & \multicolumn{2}{c|}{Place high p.}       & \multicolumn{2}{c|}{Place low p.}        & \multicolumn{2}{c|}{Polish}              & \multicolumn{2}{c|}{Span heavy}          & \multicolumn{2}{c|}{Span Light}          & \multicolumn{2}{c|}{Table}               & \multicolumn{2}{c|}{Average}             \\ \hline
\multicolumn{1}{|c|}{\textit{msec}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} \\ \hline
\multicolumn{1}{|c|}{MSR-GCN}       & 54.8               & 109.8               & 32.3               & 55.5                & \textbf{14.6}      & \textbf{26.9}       & 52.6               & 90.2                & 16.1               & 29.3                & 57.9               & 89.7                & \textbf{20.7}      & \textbf{36.1}       & \textbf{27.9}      & \textbf{47.5}       & 18.1               & 31.4                & 37.7               & 62.3                & 30.4               & \textbf{43.0}       & 53.6               & 95.4                & 34.7               & 59.8                \\
\multicolumn{1}{|c|}{DCT-RNN-GCN}   & 40.5               & 70.1                & 36.3               & 50.4                & 19.2               & 32.3                & 38.7               & 84.8                & 16.3               & \textbf{14.1}       & 51.1               & 105.5               & 35.2               & 45.9                & 39.3               & 57.9                & 16.9               & \textbf{26.9}       & 36.4               & 73.4                & 28.1               & 49.2                & 47.4               & 103.6               & 34.0               & 59.8                \\
\multicolumn{1}{|c|}{STS-GCN}       & \textbf{32.5}      & 67.8                & \textbf{27.5}      & \textbf{50.0}       & 18.2               & 41.3                & 34.7               & 79.9                & 17.2               & 32.2                & \textbf{38.9}      & 94.1                & 28.4               & 51.2                & 30.6               & 61.9                & 16.0               & 33.3                & 30.8               & 62.5                & \textbf{27.2}      & 47.7                & 35.6               & 83.5                & 28.1               & 58.7                \\ \hline
\multicolumn{1}{|c|}{Ours}          & \textbf{32.5}      & \textbf{65.4}       & 28.4               & 52.0                & 16.8               & 37.7                & \textbf{33.6}      & \textbf{75.5}       & \textbf{15.3}      & 31.7                & 40.3               & \textbf{83.8}       & 27.8               & 52.0                & 30.4               & 59.6                & \textbf{15.3}      & 31.0                & \textbf{30.2}      & \textbf{62.0}       & 28.8               & 57.3                & \textbf{35.3}      & \textbf{79.2}       & \textbf{27.9}      & \textbf{57.3}       \\ \hline
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}

==> tab/tab_vecchie/h36m_ablative.tex <==
\begin{table}[!ht]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{|c|cc|c|}
\cline{2-3}
\multicolumn{1}{c|}{}     & \multicolumn{2}{c}{Average}   & \multicolumn{1}{|c}{}                                 \\ 
\hline
\textit{msec} & {\ul \textit{400}} & {\ul \textit{1000}} & Parameters (k) \\ \hline
Full $\mathcal{G}^{st}$ + Conv      & 40.8               & 82.5                & 222.9          \\
Full $\mathcal{G}^{st}$ + DW-Conv   & 41.1               & 79.1                & 248.5          \\
Separable $\mathcal{G}^{s-t}$ +  Conv    & 38.3               & 75.6                & 57.5           \\
Separable $\mathcal{G}^{s-t}$  + DW-Conv & \textbf{37.6}               & \textbf{73.8}                & 83.0           \\ \hline
\end{tabular}}
\caption{Comparison of ablative variants of our model. Average MPJPE error in mm on Human3.6M for short term and long term. We also report the number of parameters used for the different techniques. See Sec. \ref{subsec:ablation} for a discussion.}
\label{tab:h36m_ablation}
\end{table}

==> tab/tab_vecchie/h36m_quantitative_full.tex <==
%%% SHORT TERM MPJPE
\begin{table}[!b]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{}               & \multicolumn{2}{c|}{Walking}             & \multicolumn{2}{c|}{Eating}              & \multicolumn{2}{c|}{Smoking}             & \multicolumn{2}{c|}{Discussion}          & \multicolumn{2}{c|}{Directions}          & \multicolumn{2}{c|}{Greeting}            & \multicolumn{2}{c|}{Phoning}             & \multicolumn{2}{c|}{Posing}              \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 39.8               & 58.1                & 36.2               & 75.5                & 36.4               & 69.5                & 65.4               & 119.8               & 56.5               & 106.5               & 78.1               & 138.8               & 49.2               & 105.0               & 75.8               & 178.2               \\
\multicolumn{1}{|c|}{MSR-GCN \cite{Dang21}}        & 45.2               & 63.0                & 40.4               & 77.1                & 38.1               & 71.6                & 69.7               & 117.5               & 53.8               & 100.5               & 93.3               & 147.2               & 51.2               & 104.3               & 85.0               & 174.3               \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & 32.9               & 51.8                & 25.4               & 52.4                & 25.8               & 50.0                & 40.2               & 78.8                & 34.7              & 71.0                & 49.2               & \textbf{91.6}                & 30.9               & 66.1                & 45.6               & 106.4               \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}         
& \textbf{31.5}      & \textbf{50.1}       & \textbf{24.1}      & \textbf{48.8}       & \textbf{24.4}      & \textbf{47.7}       & \textbf{39.1}      & \textbf{76.8}       & \textbf{32.7}      & \textbf{68.5}       & \textbf{47.5}      & 91.7       & \textbf{29.7}      & \textbf{64.3}       & \textbf{44.4}      & \textbf{101.8}      \\ \hline
\end{tabular}}
\end{table}  
%\vspace{-1.3cm}
\begin{table}[!b]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{\textbf{}}      & \multicolumn{2}{c|}{Purchases}           & \multicolumn{2}{c|}{Sitting}             & \multicolumn{2}{c|}{Sitting Down}        & \multicolumn{2}{c|}{Taking Photo}        & \multicolumn{2}{c|}{Waiting}             & \multicolumn{2}{c|}{Walking Dog}         & \multicolumn{2}{c|}{Walking Together}    & \multicolumn{2}{c|}{Average}             \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 73.9               & 134.2               & 56.0               & 115.9               & 72.0               & 143.6               & 51.5               & 115.9               & 54.9               & 108.2               & 86.3               & 146.9               & 41.9               & 64.9                & 58.3               & 112.1               \\
\multicolumn{1}{|c|}{MSR-GCN \cite{Dang21}}        & 79.6               & 139.1               & 57.8               & 120.0               & 76.8               & 155.4               & 56.3               & 121.8               & 59.2               & 106.2               & 93.3               & 148.2               & 43.8               & 65.9                & 62.9               & 114.1               \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & 48.7               & 93.5                & 35.0               & 75.2                & 47.9               & 94.3                & 33.6               & 76.9                & 35.2               & 72.0                & 59.6               & 102.6               & 30.5               & 51.1       & 38.3               & 75.6                \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}        
& \textbf{47.3}      & \textbf{90.0}       & \textbf{33.8}      & \textbf{71.6}       & \textbf{46.7}      & \textbf{91.3}       & \textbf{32.4}      & \textbf{72.3}       & \textbf{32.7}      & \textbf{68.6}       & \textbf{57.7}      & \textbf{99.0}      & \textbf{29.2}      & \textbf{50.8}                & \textbf{36.9}      & \textbf{72.9}       \\ \hline
\end{tabular}}
\caption{MPJPE error in mm for short-term (400 msec, 10 frames) and long-term (1000 msec, 25 frames) predictions of 3D joint positions on Human3.6M. The proposed model outperforms the current state-of-the-art STS-GCN~\cite{stsgcn} on both horizons for each action. 
Average improvements are similar for 10 and 25 frames, 3.7\% and 3.6\% respectively.
%Average improvements are 3.7\% for 10 frames and 3.6\% for 25 frames.
%and \textit{\FG{Alessio: which one? you mention in sec 5.2 that we go up to 6.9}}, respectively of 6\% and \FG{Alessio: which one scores 6.9?}\%.
See Sec.~\ref{subsec:comparison_h36m} for the discussion. 
%\MC{uniformare SES-GCN VS ours}.
%Lowest errors in mm for aperiodic actions such as \textit{Eating} and \textit{Smoking}.
}
%\label{tab:h36m_quantitative_full}

\end{table}

==> tab/tab_vecchie/h36m_quantitative_full_ADJUSTED.tex <==
%%% SHORT TERM MPJPE
\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{}               & \multicolumn{2}{c|}{Walking}             & \multicolumn{2}{c|}{Eating}              & \multicolumn{2}{c|}{Smoking}             & \multicolumn{2}{c|}{Discussion}          & \multicolumn{2}{c|}{Directions}          & \multicolumn{2}{c|}{Greeting}            & \multicolumn{2}{c|}{Phoning}             & \multicolumn{2}{c|}{Posing}              \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 39.8               & 58.1                & 36.2               & 75.5                & 36.4               & 69.5                & 65.4               & 119.8               & 56.5               & 106.5               & 78.1               & 138.8               & 49.2               & 105.0               & 75.8               & 178.2               \\
\multicolumn{1}{|c|}{MSRGCN \cite{Dang21}}        & 45.2               & 63.0                & 40.4               & 77.1                & 38.1               & 71.6                & 69.7               & 117.5               & 53.8               & 100.5               & 93.3               & 147.2               & 51.2               & 104.3               & 85.0               & 174.3               \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & 53.3               & 70.2                & 44.3               & 82.6                & 44.6               & 76.1                & 71.2               & 118.8                & 64.0              & 109.5                & 85.9               & 136.1                & 55.3               & 108.2                & 89.1               & 178.4               \\ \hline
\multicolumn{1}{|c|}{Ours}         
& \textbf{32.0}      & \textbf{50.8}       & \textbf{24.5}      & \textbf{48.6}       & \textbf{24.5}      & \textbf{47.6}       & \textbf{39.0}      & \textbf{77.5}       & \textbf{33.4}      & \textbf{68.3}       & \textbf{48.5}      & \textbf{90.9}       & \textbf{29.8}      & \textbf{63.7}       & \textbf{43.9}      & \textbf{102.4}      \\ \hline
       

\end{tabular}}
\end{table*}  
\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{\textbf{}}      & \multicolumn{2}{c|}{Purchases}           & \multicolumn{2}{c|}{Sitting}             & \multicolumn{2}{c|}{Sitting Down}        & \multicolumn{2}{c|}{Taking Photo}        & \multicolumn{2}{c|}{Waiting}             & \multicolumn{2}{c|}{Walking Dog}         & \multicolumn{2}{c|}{Walking Together}    & \multicolumn{2}{c|}{Average}             \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 73.9               & 134.2               & 56.0               & 115.9               & 72.0               & 143.6               & 51.5               & 115.9               & 54.9               & 108.2               & 86.3               & 146.9               & 41.9               & 64.9                & 58.3               & 112.1               \\
\multicolumn{1}{|c|}{MSRGCN \cite{Dang21}}        & 79.6               & 139.1               & 57.8               & 120.0               & 76.8               & 155.4               & 56.3               & 121.8               & 59.2               & 106.2               & 93.3               & 148.2               & 43.8               & 65.9                & 62.9               & 114.1               \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & 85.9               & 141.0              & 63.9               & 121.3               & 81.5               & 148.4                & 63.4               & 126.2                & 63.3               & 113.5                & 96.0              & 151.4              & 49.8               & 72.5       & 67.4               & 116.9                \\ \hline


\multicolumn{1}{|c|}{Ours Adjusted}        
& \textbf{83.8}      & \textbf{139.4}       & \textbf{61.2}      & \textbf{118.4}       & \textbf{80.2}      & \textbf{145.6}       & \textbf{58.5}      & \textbf{121.0}       & \textbf{61.4}      & \textbf{109.5}       & \textbf{95.1}      & \textbf{149.2}      & \textbf{49.5}      & \textbf{71.1}                & \textbf{65.6}      & \textbf{114.7}       \\ \hline
\end{tabular}}
\caption{MPJPE error in mm for short-term (400 msec, 10 frames) and long-term (1000 msec, 25 frames) prediction of 3D joint positions on Human3.6M. The proposed model outperforms the current state-of-the-art \cite{stsgcn} in both the short and long term for each action. For aperiodic actions we obtain the lowest errors in terms of millimeters, such as Eating or Smoking. Over a time horizon of 10 frames there is on average an increase of 2.7\% \textit{wrt} the current best technique, while for 25 predicted frames there is a margin of improvement up to 8\%, e.g. Taking Photo. See Sec.~\ref{subsec:comparison_h36m} for the discussion.}
\label{tab:h36m_quantitative_full}
\vspace{-0.5cm}
\end{table*}

==> tab/tab_vecchie/model_construction.tex <==
\begin{table}[b]
\vspace{-0.5cm}
\centering
\resizebox{.48\textwidth}{!}{
\begin{tabular}{l|c|c|c|}
\cline{2-4}
\multicolumn{1}{l|}{}                                      & \# Layers & MPJPE                 & Parameters (k)        \\ \hline
\multicolumn{1}{|l|}{GCN}      & 4         & 81.7     & 222.7                 \\ \hline

\multicolumn{1}{|l|}{STSGCN \cite{stsgcn}}                               & 4         & 75.6                  & \textbf{57.6}                  \\
\multicolumn{1}{|l|}{ Deeper STSGCN}     & 5 & 75.1         & 68.6                  \\ 
\multicolumn{1}{|l|}{Deeper STSGCN}     & 6  & 76.1         & 79.9                  \\ \hline
\multicolumn{1}{|l|}{STSGCN + MLP}    & 5+5   & 80.9     & 101.4                 \\
\multicolumn{1}{|l|}{STSGCN+DW+MLP} & 5+5  & \underline{73.6} & 70.0                  \\ \hline
\multicolumn{1}{|l|}{STSGCN+DW+ Sparse \cite{shi21}} & 5+5  & 74.8                  & 122.4                  \\
\multicolumn{1}{|l|}{SeS-GCN (proposed)} & 5+5  & \textbf{72.9}       & \underline{58.6}               \\ \hline
\end{tabular}}
\caption{MPJPE error (millimeters) for long-range predictions (25 frames) on Human3.6M \cite{h36m_pami}  and number of parameters for the different implementations involved in building our model. Our final model outperforms the current state-of-the-art \cite{stsgcn} by 3.6\% while using only 85.5\% parameters. See \ref{subsec:model_choices} for discussion.}
\label{tab:model_table}
\end{table}

==> tab/tab_vecchie/model_construction_NEW.tex <==
\begin{table}[b]
\vspace{-0.5cm}
\centering
\resizebox{.48\textwidth}{!}{
\begin{tabular}{l|c|c|c|}
\cline{2-4}
\multicolumn{1}{l|}{}                                      & \# Layers & MPJPE                 & Parameters (k)        \\ \hline
\multicolumn{1}{|l|}{GCN}      & 4         & 81.7     & 222.7                 \\ \hline


\multicolumn{1}{|l|}{DW-GCN [cite DW]}                               & 4+4         & 79.0                  & 223.2                  \\
\multicolumn{1}{|l|}{STS-GCN [cite STS]}     & 4 & 75.6         & \textbf{57.6}                  \\ 
\multicolumn{1}{|l|}{Sparse-GCN [cite SGCN]}     & 4  & 79.3         & 205.9 (257.9)                  \\ \hline



\multicolumn{1}{|l|}{Deeper STSGCN}     & 5 & 75.1         & 68.6                  \\ 
\multicolumn{1}{|l|}{Deeper STSGCN}     & 6  & 76.1         & 79.9                  \\ \hline


\multicolumn{1}{|l|}{STSGCN + MLP}    & 5+5   & 80.9     & 101.4                 \\
\multicolumn{1}{|l|}{STSGCN+DW+MLP} & 5+5  & \underline{73.6} & 70.0                  \\ \hline


\multicolumn{1}{|l|}{STSGCN+DW+ Sparse \cite{shi21}} & 5+5  & 74.8                  & 122.4                  \\
\multicolumn{1}{|l|}{SeS-GCN (proposed)} & 5+5  & \textbf{72.9}       & \underline{58.6}               \\ \hline
\end{tabular}}
\caption{MPJPE error (millimeters) for long-range predictions (25 frames) on Human3.6M \cite{h36m_pami}  and number of parameters for the different implementations involved in building our model. Our final model outperforms the current state-of-the-art \cite{stsgcn} by 3.6\% while using only 85.5\% parameters. See \ref{subsec:model_choices} for discussion.}
\label{tab:model_table}
\end{table}

==> tab/tab_vecchie/symb_quantitative_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-15}
                                    & \multicolumn{2}{c|}{Crash heavy}         & \multicolumn{2}{c|}{Crash light}         & \multicolumn{2}{c|}{Crash polish}        & \multicolumn{2}{c|}{Ground}              & \multicolumn{2}{c|}{Hammer}              & \multicolumn{2}{c|}{Lift}                & \multicolumn{2}{c|}{Place high p.}       \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 40.5               & 70.1                & 36.3               & 50.4                & 19.2               & 32.3                & 38.7               & 84.8                & 16.3               & \textbf{14.1}       & 51.1               & 105.5               & 35.2               & 45.9                \\
\multicolumn{1}{|c|}{MSRGCN \cite{Dang21}}       & 53.4               & 109.8               & 29.6               & 55.5                & \textbf{13.7}      & \textbf{26.9}       & 51.1               & 90.2                & \textbf{14.3}      & 29.3                & 56.3               & 89.7                & \textbf{19.6}      & \textbf{36.1}       \\

\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & \textbf{32.5}      & 67.8                & \textbf{27.5}      & \textbf{50.0}       & 18.2               & 41.3                & 34.7               & 79.9                & 17.2               & 32.2                & \textbf{38.9}      & 94.1                & 28.4               & 51.2                \\ \hline
\multicolumn{1}{|c|}{Ours}          & \textbf{32.5}      & \textbf{65.4}       & 28.4               & 52.0                & 16.8               & 37.7                & \textbf{33.6}      & \textbf{75.5}       & 15.3               & 31.7                & 40.3               & \textbf{83.8}       & 27.8               & 52.0                \\ \hline
\end{tabular}}
\end{table*}


\begin{table*}[!htb]
\centering
\resizebox{.9\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|}
\cline{2-13}
                                    & \multicolumn{2}{c|}{Place low p.}        & \multicolumn{2}{c|}{Polish}              & \multicolumn{2}{c|}{Span heavy}          & \multicolumn{2}{c|}{Span Light}          & \multicolumn{2}{c|}{Table}               & \multicolumn{2}{c|}{Average}             \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} & {\ul \textit{660}} & {\ul \textit{1660}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}   & 39.3               & 57.9                & 16.9               & \textbf{26.9}       & 36.4               & 73.4                & 28.1               & 49.2                & 47.4               & 103.6               & 34.0               & 59.8                \\
\multicolumn{1}{|c|}{MSRGCN \cite{Dang21}}       & \textbf{26.8}      & \textbf{47.5}       & 17.0               & 31.4                & 36.4               & 62.3                & 29.3               & \textbf{43.0}       & 52.4               & 95.4                & 33.3               & 59.8                \\

\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}       & 30.6               & 61.9                & 16.0               & 33.3                & 30.8               & 62.5                & \textbf{27.2}      & 47.7                & 35.6               & 83.5                & 28.1               & 58.7                \\ \hline
\multicolumn{1}{|c|}{Ours}          & 30.4               & 59.6                & \textbf{15.3}      & 31.0                & \textbf{30.2}      & \textbf{62.0}       & 28.8               & 57.3                & \textbf{35.3}      & \textbf{79.2}       & \textbf{27.9}      & \textbf{57.3}       \\ \hline
\end{tabular}}
\caption{MPJPE error in mm for short-term (660 msec, 10 frames) and long-term (1660 msec, 25 frames) prediction of 3D joint positions on \dataname dataset. Our SeS-GCN is in line with the baselines considered for simple actions, e.g. Place low p. or Span Light. It performs particularly better for complex actions such as Ground, Lift and Table, for which two hands are required. The average error is 0.8\% lower than the other models in the short-term and 2.4\% lower in the long-term prediction. See Sec.\ref{subsec:quantitative_symb} for a discussion.}
\label{tab:quantitative_symbiotic}
\vspace{-0.5cm}
\end{table*}




==> tab/tab_vecchie/test_time.tex <==
\begin{table}[!htb]
\centering
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{c|cccc|}
\cline{2-5}
                                         & \multicolumn{1}{c|}{DCT-RNN-GCN} & \multicolumn{1}{c|}{MSRGCN} & \multicolumn{1}{c|}{STS-GCN} & Ours   \\ \hline
\multicolumn{1}{|c|}{\textit{Test time (sec)}} & $3.21 \times 10^{-2}$     & $4.93 \times 10^{-2}$ &   $4.78 \times 10^{-3}$  &  $5.02 \times 10^{-3}$ \\ \hline
\end{tabular}}
\caption{Caption}
\label{tab:test_time}
\end{table}

==> tab/tab_vecchie/test_time_vertical.tex <==
\begin{table}[h!]
\centering
\resizebox{.48\textwidth}{!}{
\begin{tabular}{c|c|c|c|}
\cline{2-4}
                                         & \multicolumn{1}{c|}{\textit{Test time (sec)}} & \multicolumn{1}{c|}{\textit{H3.6M (MPJPE)}} & \textit{CoHRE (MPJPE)} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN~\cite{Mao20DCT}}        & $3.21 \times 10^{-2}$                                    & 112.1                                       & 59.8                   \\
\multicolumn{1}{|c|}{MSRGCN~\cite{Dang21}}             & $4.93 \times 10^{-2}$                                         & 114.1                                       & 59.8                   \\
\multicolumn{1}{|c|}{STS-GCN~\cite{stsgcn}}            & $4.78 \times 10^{-3}$                                          & 75.6                                        & 58.7                   \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)} & $4.83 \times 10^{-3}$                                          & 72.9                                        & 57.3                   \\ \hline
\end{tabular}}
\caption{
Comparison of runtime of SeS-GCN against best performing competing techniques. For a complete comparison, MPJPE errors are also reported, for the predictions at 25-frame future horizons (see Tables 2 and 4\textit{(main paper)} for complete performance evaluations). The indicated runtime is the prediction time for a single future frame, performed on a remote Google Colaboratory's GPU.
See Sec.~\ref{sec:impl_det} for discussion.
%Comparison on MPJPE (we considered the average for both datsets) for long-range prediction and time employed by our model and the baselines we considered to make a forecast on a single sample. Due to its lightweight architecture our model is competitive with STS-GCN\cite{stsgcn} it requires just 0.05 additional msec, while it is faster than \cite{Mao20DCT, Dang21} by 85\% and 90.27\%, respectively. All those results were computed on Google Colaboratory's GPU. 
}
\label{tab:test_time}
\end{table}



==> tab/tab_vecchie/upd_chico_quantitative.tex <==
\begin{table}[]
\centering
\resizebox{1.\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|}
\cline{2-17}
\multicolumn{1}{l|}{}                              & \multicolumn{2}{c|}{Hammer}              & \multicolumn{2}{c|}{High Lift}           & \multicolumn{2}{c|}{Prec. P\&P}          & \multicolumn{2}{c|}{Rnd. P\&P}                     & \multicolumn{2}{c|}{Polishing}           & \multicolumn{2}{c|}{Heavy P\&P}          & \multicolumn{2}{c|}{Light P\&P}          & \multicolumn{2}{c|}{Average}             \\ \hline
\multicolumn{1}{|c|}{\textit{Time Horizon (msec)}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}}           & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} & {\ul \textit{400}} & {\ul \textit{1000}} \\ \hline
\multicolumn{1}{|c|}{DCT-RNN-GCN \cite{Mao20DCT}}                  & 36.0               & 35.3                & 61.9               & 113.9               & 45.0               & 74.1                & 46.6                         & 78.1                & 37.4               & 67.1                & 56.7               & 106.7               & 54.7               & 92.4                & 48.4               & 81.1                \\
\multicolumn{1}{|c|}{MSR-GCN \cite{Dang21}}                       & \textbf{34.1}      & \textbf{32.0}       & 78.4               & 151.7               & 51.4               & 88.8                & 52.6 & 92.2                & \textbf{36.7}      & \textbf{64.2}       & 66.2               & 128.3               & 66.2               & 117.5               & 55.1               & 96.4                \\
\multicolumn{1}{|c|}{STS-GCN \cite{stsgcn}}                      & 47.4               & 63.1                & 59.8               & 106.8               & 43.3               & 70.9                & 46.4                         & 76.1                & 39.2               & 68.4                & 53.8               & \textbf{90.5}       & 51.4               & 83.5                & 48.7               & 79.9                \\ \hline
\multicolumn{1}{|c|}{SeS-GCN (proposed)}           & 41.4               & 51.8                & \textbf{57.9}      & \textbf{103.3}      & \textbf{42.0}      & \textbf{69.7}       & \textbf{44.6}                & \textbf{73.4}       & 36.8               & 64.5                & \textbf{53.0}      & 90.7                & \textbf{50.1}      & \textbf{82.3}       & \textbf{46.6}      & \textbf{75.6}       \\ \hline
\end{tabular}
}
\caption{ MPJPE error in mm for short-term (400 msec, 10 frames) and long-term (1000 msec, 25 frames) prediction of 3D joint positions on \dataname dataset. Our SeS-GCN performs particularly better for complex actions such as High Lift and Rnd. P\emph{\&}P. The average error is 3.7\% lower than the other models in the short-term and 5.4\% lower in the long-term prediction. See Sec.\ref{subsec:quantitative_symb} for a discussion.}
\label{tab:CHICOresults}
\vspace{-.3cm}
\end{table}

%Metrics &  \textit{Recall} & \textit{Prec} & \textit{F}$_1$ & \textit{Inference Time (sec)} \\ \hline
%          \multicolumn{1}{|c|}{DCT-RNN-GCN~\cite{Mao20DCT}}& 0.80 & 0.61 & 0.70 &  $9.1 \times 10^{-3}$\\
%          \multicolumn{1}{|c|}{MSR-GCN~\cite{Dang21}}& 0.5 & 0.12 & 0.20 & $25.2 \times 10^{-3}$\\
%          \multicolumn{1}{|c|}{STS-GCN~\cite{stsgcn}}& 0.81 & 0.69 & 0.74 & {$\mathbf{2.3 \times 10^{-3}}$} \\ \hline
%          \multicolumn{1}{|c|}{SeS-GCN (proposed)} & 0.86 & 0.66 & \textbf{0.75} & {$\mathbf{2.3 \times 10^{-3}}$}\\ \hline

==> tab/vertical_comparison_dataset.tex <==
\begin{table}[!h]
\centering

\begin{tabular}{c|c|c|}
\cline{2-3}
\multicolumn{1}{l|}{\textbf{}}       & Symbiotic:Human & Human3.6M  \\ \hline
\multicolumn{1}{|c|}{N° of actions}  & 12              & 15         \\
\multicolumn{1}{|c|}{N° of actors}   & 8               & 7          \\
\multicolumn{1}{|c|}{N° of frames}   & 70K             & 3.6M       \\
\multicolumn{1}{|c|}{N° of keypoint} & 18              & 32         \\
\multicolumn{1}{|c|}{Framerate}      & 15              & 25         \\
\multicolumn{1}{|c|}{Aspect Ratio}   & Not normalized  & Normalized \\
\multicolumn{1}{|c|}{Fine grained}   & Yes             & No         \\ \hline
\end{tabular}
\caption{Comparison of the two datasets showing the main differences. The actions in the symbiotic dataset are purely task-specific, without any movement that is not inherent to the action. This influences the lower number of frames compared to Human 3.6M. \fab{What about the comparison with [4,11,12,15]? We write it in Sec 4.} \fab{The no. frames seems a killer for our symbiotic.. may we read data in a different way and avoid this inconvenient comparison?} \ale{could I suggest recording time for each actor..? Does this make sense?}}
\label{tab:vertical_symbiotic_h36_comparative}
\end{table}
